Extended Report: The Implicit Calculus

Generic programming (GP) is an increasingly important trend in programming languages. Well-known GP mechanisms, such as type classes and the C++0x concepts proposal, usually combine two features: 1) a special type of interfaces; and 2) implicit instantiation of implementations of those interfaces. Scala implicits are a GP language mechanism, inspired by type classes, that break with the tradition of coupling implicit instantiation with a special type of interface. Instead, implicits provide only implicit instantiation, which is generalized to work for any types. This turns out to be quite powerful and useful to address many limitations that show up in other GP mechanisms. This paper synthesizes the key ideas of implicits formally in a minimal and general core calculus called the implicit calculus, and it shows how to build source languages supporting implicit instantiation on top of it. A novelty of the calculus is its support for partial resolution and higher-order rules (a feature that has been proposed before, but was never formalized or implemented). Ultimately, the implicit calculus provides a formal model of implicits, which can be used by language designers to study and inform implementations of similar mechanisms in their own languages.

==> Preamble.tex <==
%%include lhs2TeX.fmt
%% ODER: format ==         = "\mathrel{==}"
%% ODER: format /=         = "\neq "
%
%
\makeatletter
\@ifundefined{lhs2tex.lhs2tex.sty.read}%
  {\@namedef{lhs2tex.lhs2tex.sty.read}{}%
   \newcommand\SkipToFmtEnd{}%
   \newcommand\EndFmtInput{}%
   \long\def\SkipToFmtEnd#1\EndFmtInput{}%
  }\SkipToFmtEnd

\newcommand\ReadOnlyOnce[1]{\@ifundefined{#1}{\@namedef{#1}{}}\SkipToFmtEnd}
\usepackage{amstext}
\usepackage{amssymb}
\usepackage{stmaryrd}
\DeclareFontFamily{OT1}{cmtex}{}
\DeclareFontShape{OT1}{cmtex}{m}{n}
  {<5><6><7><8>cmtex8
   <9>cmtex9
   <10><10.95><12><14.4><17.28><20.74><24.88>cmtex10}{}
\DeclareFontShape{OT1}{cmtex}{m}{it}
  {<-> ssub * cmtt/m/it}{}
\newcommand{\texfamily}{\fontfamily{cmtex}\selectfont}
\DeclareFontShape{OT1}{cmtt}{bx}{n}
  {<5><6><7><8>cmtt8
   <9>cmbtt9
   <10><10.95><12><14.4><17.28><20.74><24.88>cmbtt10}{}
\DeclareFontShape{OT1}{cmtex}{bx}{n}
  {<-> ssub * cmtt/bx/n}{}
\newcommand{\tex}[1]{\text{\texfamily#1}}	% NEU

\newcommand{\Sp}{\hskip.33334em\relax}


\newcommand{\Conid}[1]{\mathit{#1}}
\newcommand{\Varid}[1]{\mathit{#1}}
\newcommand{\anonymous}{\kern0.06em \vbox{\hrule\@width.5em}}
\newcommand{\plus}{\mathbin{+\!\!\!+}}
\newcommand{\bind}{\mathbin{>\!\!\!>\mkern-6.7mu=}}
\newcommand{\rbind}{\mathbin{=\mkern-6.7mu<\!\!\!<}}% suggested by Neil Mitchell
\newcommand{\sequ}{\mathbin{>\!\!\!>}}
\renewcommand{\leq}{\leqslant}
\renewcommand{\geq}{\geqslant}
\usepackage{polytable}

%mathindent has to be defined
\@ifundefined{mathindent}%
  {\newdimen\mathindent\mathindent\leftmargini}%
  {}%

\def\resethooks{%
  \global\let\SaveRestoreHook\empty
  \global\let\ColumnHook\empty}
\newcommand*{\savecolumns}[1][default]%
  {\g@addto@macro\SaveRestoreHook{\savecolumns[#1]}}
\newcommand*{\restorecolumns}[1][default]%
  {\g@addto@macro\SaveRestoreHook{\restorecolumns[#1]}}
\newcommand*{\aligncolumn}[2]%
  {\g@addto@macro\ColumnHook{\column{#1}{#2}}}

\resethooks

\newcommand{\onelinecommentchars}{\quad-{}- }
\newcommand{\commentbeginchars}{\enskip\{-}
\newcommand{\commentendchars}{-\}\enskip}

\newcommand{\visiblecomments}{%
  \let\onelinecomment=\onelinecommentchars
  \let\commentbegin=\commentbeginchars
  \let\commentend=\commentendchars}

\newcommand{\invisiblecomments}{%
  \let\onelinecomment=\empty
  \let\commentbegin=\empty
  \let\commentend=\empty}

\visiblecomments

\newlength{\blanklineskip}
\setlength{\blanklineskip}{0.66084ex}

\newcommand{\hsindent}[1]{\quad}% default is fixed indentation
\let\hspre\empty
\let\hspost\empty
\newcommand{\NB}{\textbf{NB}}
\newcommand{\Todo}[1]{$\langle$\textbf{To do:}~#1$\rangle$}

\EndFmtInput
\makeatother
%
%
%
%
%
%
% This package provides two environments suitable to take the place
% of hscode, called "plainhscode" and "arrayhscode". 
%
% The plain environment surrounds each code block by vertical space,
% and it uses \abovedisplayskip and \belowdisplayskip to get spacing
% similar to formulas. Note that if these dimensions are changed,
% the spacing around displayed math formulas changes as well.
% All code is indented using \leftskip.
%
% Changed 19.08.2004 to reflect changes in colorcode. Should work with
% CodeGroup.sty.
%
\ReadOnlyOnce{polycode.fmt}%
\makeatletter

\newcommand{\hsnewpar}[1]%
  {{\parskip=0pt\parindent=0pt\par\vskip #1\noindent}}

% can be used, for instance, to redefine the code size, by setting the
% command to \small or something alike
\newcommand{\hscodestyle}{}

% The command \sethscode can be used to switch the code formatting
% behaviour by mapping the hscode environment in the subst directive
% to a new LaTeX environment.

\newcommand{\sethscode}[1]%
  {\expandafter\let\expandafter\hscode\csname #1\endcsname
   \expandafter\let\expandafter\endhscode\csname end#1\endcsname}

% "compatibility" mode restores the non-polycode.fmt layout.

\newenvironment{compathscode}%
  {\par\noindent
   \advance\leftskip\mathindent
   \hscodestyle
   \let\\=\@normalcr
   \(\pboxed}%
  {\endpboxed\)%
   \par\noindent
   \ignorespacesafterend}

\newcommand{\compaths}{\sethscode{compathscode}}

% "plain" mode is the proposed default.

\newenvironment{plainhscode}%
  {\hsnewpar\abovedisplayskip
   \advance\leftskip\mathindent
   \hscodestyle
   \let\\=\@normalcr
   \(\pboxed}%
  {\endpboxed\)%
   \hsnewpar\belowdisplayskip
   \ignorespacesafterend}

% Here, we make plainhscode the default environment.

\newcommand{\plainhs}{\sethscode{plainhscode}}
\plainhs

% The arrayhscode is like plain, but makes use of polytable's
% parray environment which disallows page breaks in code blocks.

\newenvironment{arrayhscode}%
  {\hsnewpar\abovedisplayskip
   \advance\leftskip\mathindent
   \hscodestyle
   \let\\=\@normalcr
   \(\parray}%
  {\endparray\)%
   \hsnewpar\belowdisplayskip
   \ignorespacesafterend}

\newcommand{\arrayhs}{\sethscode{arrayhscode}}

% The mathhscode environment also makes use of polytable's parray 
% environment. It is supposed to be used only inside math mode 
% (I used it to typeset the type rules in my thesis).

\newenvironment{mathhscode}%
  {\parray}{\endparray}

\newcommand{\mathhs}{\sethscode{mathhscode}}

% texths is similar to mathhs, but works in text mode.

\newenvironment{texthscode}%
  {\(\parray}{\endparray\)}

\newcommand{\texths}{\sethscode{texthscode}}

% The framed environment places code in a framed box.

\def\codeframewidth{\arrayrulewidth}
\RequirePackage{calc}

\newenvironment{framedhscode}%
  {\parskip=\abovedisplayskip\par\noindent
   \hscodestyle
   \arrayrulewidth=\codeframewidth
   \tabular{@{}|p{\linewidth-2\arraycolsep-2\arrayrulewidth-2pt}|@{}}%
   \hline\framedhslinecorrect\\{-1.5ex}%
   \let\endoflinesave=\\
   \let\\=\@normalcr
   \(\pboxed}%
  {\endpboxed\)%
   \framedhslinecorrect\endoflinesave{.5ex}\hline
   \endtabular
   \parskip=\belowdisplayskip\par\noindent
   \ignorespacesafterend}

\newcommand{\framedhslinecorrect}[2]%
  {#1[#2]}

\newcommand{\framedhs}{\sethscode{framedhscode}}

% The inlinehscode environment is an experimental environment
% that can be used to typeset displayed code inline.

\newenvironment{inlinehscode}%
  {\(\def\column##1##2{}%
   \let\>\undefined\let\<\undefined\let\\\undefined
   \newcommand\>[1][]{}\newcommand\<[1][]{}\newcommand\\[1][]{}%
   \def\fromto##1##2##3{##3}%
   \def\nextline{}}{\) }%

\newcommand{\inlinehs}{\sethscode{inlinehscode}}

% The joincode environment is a separate environment that
% can be used to surround and thereby connect multiple code
% blocks.

\newenvironment{joincode}%
  {\let\orighscode=\hscode
   \let\origendhscode=\endhscode
   \def\endhscode{\def\hscode{\endgroup\def\@currenvir{hscode}\\}\begingroup}
   %\let\SaveRestoreHook=\empty
   %\let\ColumnHook=\empty
   %\let\resethooks=\empty
   \orighscode\def\hscode{\endgroup\def\@currenvir{hscode}}}%
  {\origendhscode
   \global\let\hscode=\orighscode
   \global\let\endhscode=\origendhscode}%

\makeatother
\EndFmtInput
%

==> src/Abs.tex <==
Implicit programming that infers values by using type
information has proven its benefits in practice. However, 
years of experience have exposed several limitations in its current practice.
For example, Haskell's type classes, which are the oldest and most
prominent form of implicit programming have several
limitations of its original design: no
ability to control the \emph{scoping} of instances; the \emph{second
  class} nature of types classes compared to types; and type class
constraints being limited to \emph{first-order predicates}.

This paper presents a \textit{implicit calculus}: a powerful and expressive,
yet minimalistic, calculus that provides an implicit programming model
without the limitations of the current practice. The implicit calculus
offers control over scoping, does not suffer from the second class
nature of type classes, and incoorporates two features which
have been discussed in the literature but for which there is
currently no good solution: \emph{higher-order predicates} and
\emph{coherent support for overlapping instances}.  We present the
syntax, operational semantics, type system, type-directed translation
into System F, as well as correctness results. Finally, we show how
Haskell and Scala's implicit programming constructs are translated
into our calculus.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../Main"
%%% End: 


==> src/Intro.tex <==
%% ODER: format ==         = "\mathrel{==}"
%% ODER: format /=         = "\neq "
%
%
\makeatletter
\@ifundefined{lhs2tex.lhs2tex.sty.read}%
  {\@namedef{lhs2tex.lhs2tex.sty.read}{}%
   \newcommand\SkipToFmtEnd{}%
   \newcommand\EndFmtInput{}%
   \long\def\SkipToFmtEnd#1\EndFmtInput{}%
  }\SkipToFmtEnd

\newcommand\ReadOnlyOnce[1]{\@ifundefined{#1}{\@namedef{#1}{}}\SkipToFmtEnd}
\usepackage{amstext}
\usepackage{amssymb}
\usepackage{stmaryrd}
\DeclareFontFamily{OT1}{cmtex}{}
\DeclareFontShape{OT1}{cmtex}{m}{n}
  {<5><6><7><8>cmtex8
   <9>cmtex9
   <10><10.95><12><14.4><17.28><20.74><24.88>cmtex10}{}
\DeclareFontShape{OT1}{cmtex}{m}{it}
  {<-> ssub * cmtt/m/it}{}
\newcommand{\texfamily}{\fontfamily{cmtex}\selectfont}
\DeclareFontShape{OT1}{cmtt}{bx}{n}
  {<5><6><7><8>cmtt8
   <9>cmbtt9
   <10><10.95><12><14.4><17.28><20.74><24.88>cmbtt10}{}
\DeclareFontShape{OT1}{cmtex}{bx}{n}
  {<-> ssub * cmtt/bx/n}{}
\newcommand{\tex}[1]{\text{\texfamily#1}}	% NEU

\newcommand{\Sp}{\hskip.33334em\relax}


\newcommand{\Conid}[1]{\mathit{#1}}
\newcommand{\Varid}[1]{\mathit{#1}}
\newcommand{\anonymous}{\kern0.06em \vbox{\hrule\@width.5em}}
\newcommand{\plus}{\mathbin{+\!\!\!+}}
\newcommand{\bind}{\mathbin{>\!\!\!>\mkern-6.7mu=}}
\newcommand{\rbind}{\mathbin{=\mkern-6.7mu<\!\!\!<}}% suggested by Neil Mitchell
\newcommand{\sequ}{\mathbin{>\!\!\!>}}
\renewcommand{\leq}{\leqslant}
\renewcommand{\geq}{\geqslant}
\usepackage{polytable}

%mathindent has to be defined
\@ifundefined{mathindent}%
  {\newdimen\mathindent\mathindent\leftmargini}%
  {}%

\def\resethooks{%
  \global\let\SaveRestoreHook\empty
  \global\let\ColumnHook\empty}
\newcommand*{\savecolumns}[1][default]%
  {\g@addto@macro\SaveRestoreHook{\savecolumns[#1]}}
\newcommand*{\restorecolumns}[1][default]%
  {\g@addto@macro\SaveRestoreHook{\restorecolumns[#1]}}
\newcommand*{\aligncolumn}[2]%
  {\g@addto@macro\ColumnHook{\column{#1}{#2}}}

\resethooks

\newcommand{\onelinecommentchars}{\quad-{}- }
\newcommand{\commentbeginchars}{\enskip\{-}
\newcommand{\commentendchars}{-\}\enskip}

\newcommand{\visiblecomments}{%
  \let\onelinecomment=\onelinecommentchars
  \let\commentbegin=\commentbeginchars
  \let\commentend=\commentendchars}

\newcommand{\invisiblecomments}{%
  \let\onelinecomment=\empty
  \let\commentbegin=\empty
  \let\commentend=\empty}

\visiblecomments

\newlength{\blanklineskip}
\setlength{\blanklineskip}{0.66084ex}

\newcommand{\hsindent}[1]{\quad}% default is fixed indentation
\let\hspre\empty
\let\hspost\empty
\newcommand{\NB}{\textbf{NB}}
\newcommand{\Todo}[1]{$\langle$\textbf{To do:}~#1$\rangle$}

\EndFmtInput
\makeatother
%
%
%
% First, let's redefine the forall, and the dot.
%
%
% This is made in such a way that after a forall, the next
% dot will be printed as a period, otherwise the formatting
% of `comp_` is used. By redefining `comp_`, as suitable
% composition operator can be chosen. Similarly, period_
% is used for the period.
%
\ReadOnlyOnce{forall.fmt}%
\makeatletter

% The HaskellResetHook is a list to which things can
% be added that reset the Haskell state to the beginning.
% This is to recover from states where the hacked intelligence
% is not sufficient.

\let\HaskellResetHook\empty
\newcommand*{\AtHaskellReset}[1]{%
  \g@addto@macro\HaskellResetHook{#1}}
\newcommand*{\HaskellReset}{\HaskellResetHook}

\global\let\hsforallread\empty

\newcommand\hsforall{\global\let\hsdot=\hsperiodonce}
\newcommand*\hsperiodonce[2]{#2\global\let\hsdot=\hscompose}
\newcommand*\hscompose[2]{#1}

\AtHaskellReset{\global\let\hsdot=\hscompose}

% In the beginning, we should reset Haskell once.
\HaskellReset

\makeatother
\EndFmtInput
%
%
%
%
%
% This package provides two environments suitable to take the place
% of hscode, called "plainhscode" and "arrayhscode". 
%
% The plain environment surrounds each code block by vertical space,
% and it uses \abovedisplayskip and \belowdisplayskip to get spacing
% similar to formulas. Note that if these dimensions are changed,
% the spacing around displayed math formulas changes as well.
% All code is indented using \leftskip.
%
% Changed 19.08.2004 to reflect changes in colorcode. Should work with
% CodeGroup.sty.
%
\ReadOnlyOnce{polycode.fmt}%
\makeatletter

\newcommand{\hsnewpar}[1]%
  {{\parskip=0pt\parindent=0pt\par\vskip #1\noindent}}

% can be used, for instance, to redefine the code size, by setting the
% command to \small or something alike
\newcommand{\hscodestyle}{}

% The command \sethscode can be used to switch the code formatting
% behaviour by mapping the hscode environment in the subst directive
% to a new LaTeX environment.

\newcommand{\sethscode}[1]%
  {\expandafter\let\expandafter\hscode\csname #1\endcsname
   \expandafter\let\expandafter\endhscode\csname end#1\endcsname}

% "compatibility" mode restores the non-polycode.fmt layout.

\newenvironment{compathscode}%
  {\par\noindent
   \advance\leftskip\mathindent
   \hscodestyle
   \let\\=\@normalcr
   \let\hspre\(\let\hspost\)%
   \pboxed}%
  {\endpboxed\)%
   \par\noindent
   \ignorespacesafterend}

\newcommand{\compaths}{\sethscode{compathscode}}

% "plain" mode is the proposed default.
% It should now work with \centering.
% This required some changes. The old version
% is still available for reference as oldplainhscode.

\newenvironment{plainhscode}%
  {\hsnewpar\abovedisplayskip
   \advance\leftskip\mathindent
   \hscodestyle
   \let\hspre\(\let\hspost\)%
   \pboxed}%
  {\endpboxed%
   \hsnewpar\belowdisplayskip
   \ignorespacesafterend}

\newenvironment{oldplainhscode}%
  {\hsnewpar\abovedisplayskip
   \advance\leftskip\mathindent
   \hscodestyle
   \let\\=\@normalcr
   \(\pboxed}%
  {\endpboxed\)%
   \hsnewpar\belowdisplayskip
   \ignorespacesafterend}

% Here, we make plainhscode the default environment.

\newcommand{\plainhs}{\sethscode{plainhscode}}
\newcommand{\oldplainhs}{\sethscode{oldplainhscode}}
\plainhs

% The arrayhscode is like plain, but makes use of polytable's
% parray environment which disallows page breaks in code blocks.

\newenvironment{arrayhscode}%
  {\hsnewpar\abovedisplayskip
   \advance\leftskip\mathindent
   \hscodestyle
   \let\\=\@normalcr
   \(\parray}%
  {\endparray\)%
   \hsnewpar\belowdisplayskip
   \ignorespacesafterend}

\newcommand{\arrayhs}{\sethscode{arrayhscode}}

% The mathhscode environment also makes use of polytable's parray 
% environment. It is supposed to be used only inside math mode 
% (I used it to typeset the type rules in my thesis).

\newenvironment{mathhscode}%
  {\parray}{\endparray}

\newcommand{\mathhs}{\sethscode{mathhscode}}

% texths is similar to mathhs, but works in text mode.

\newenvironment{texthscode}%
  {\(\parray}{\endparray\)}

\newcommand{\texths}{\sethscode{texthscode}}

% The framed environment places code in a framed box.

\def\codeframewidth{\arrayrulewidth}
\RequirePackage{calc}

\newenvironment{framedhscode}%
  {\parskip=\abovedisplayskip\par\noindent
   \hscodestyle
   \arrayrulewidth=\codeframewidth
   \tabular{@{}|p{\linewidth-2\arraycolsep-2\arrayrulewidth-2pt}|@{}}%
   \hline\framedhslinecorrect\\{-1.5ex}%
   \let\endoflinesave=\\
   \let\\=\@normalcr
   \(\pboxed}%
  {\endpboxed\)%
   \framedhslinecorrect\endoflinesave{.5ex}\hline
   \endtabular
   \parskip=\belowdisplayskip\par\noindent
   \ignorespacesafterend}

\newcommand{\framedhslinecorrect}[2]%
  {#1[#2]}

\newcommand{\framedhs}{\sethscode{framedhscode}}

% The inlinehscode environment is an experimental environment
% that can be used to typeset displayed code inline.

\newenvironment{inlinehscode}%
  {\(\def\column##1##2{}%
   \let\>\undefined\let\<\undefined\let\\\undefined
   \newcommand\>[1][]{}\newcommand\<[1][]{}\newcommand\\[1][]{}%
   \def\fromto##1##2##3{##3}%
   \def\nextline{}}{\) }%

\newcommand{\inlinehs}{\sethscode{inlinehscode}}

% The joincode environment is a separate environment that
% can be used to surround and thereby connect multiple code
% blocks.

\newenvironment{joincode}%
  {\let\orighscode=\hscode
   \let\origendhscode=\endhscode
   \def\endhscode{\def\hscode{\endgroup\def\@currenvir{hscode}\\}\begingroup}
   %\let\SaveRestoreHook=\empty
   %\let\ColumnHook=\empty
   %\let\resethooks=\empty
   \orighscode\def\hscode{\endgroup\def\@currenvir{hscode}}}%
  {\origendhscode
   \global\let\hscode=\orighscode
   \global\let\endhscode=\origendhscode}%

\makeatother
\EndFmtInput
%


\newcommand{\Meta}[1]{{\it #1\/}}
\newcommand{\m}[1]{\ensuremath{#1}}

\newcommand{\qlam}[2]{\m{\lambda\{#1\}.#2}}
\newcommand{\qask}[1]{\m{\Meta{?}#1}}
\newcommand{\qapp}[2]{\m{(#1)\;\texttt{with}\;#2}}
\newcommand{\qlet}[2]{\texttt{implicit}\;#1\;\texttt{in}\;#2}
\newcommand{\qLam}[2]{\m{\Lambda#1.#2}} 
  
\newcommand{\ty}[1]{\Meta{#1}}
\newcommand{\tyInt}{\Meta{int}}
\newcommand{\tyBool}{\Meta{bool}}
\newcommand{\rulety}[2]{\m{\{#1\}\!\Rightarrow\!#2}}

\section{Introduction}
\label{sec:intro}

%%* Implicit programming
%%* Type classes, C++ concepts, Scala implicits, JavaGI
%%* resolution, type-based

Implicit programming infers values by using type information. It is
``implicit'' because we can omit expressions (e.g. those for function's
parameters) and instead implicitly rely on its type-directed inference
of necessary values. 
%mentioning a type does not explicitly pinpoint a
%value by an expression but just means a value of that type.
Implicit values are either fetched by their types from
the current (implicit) environment or constructed by type-directed \emph{rules}. 

Implicit programming has proven its benefits in practice.  Haskell's
\emph{type classes}, Scala's \emph{implicits} , JavaGI, various
proposals for C++'s \emph{concepts} are all implicit programming
mechanisms. Implicit programming significantly reduces the amount of tedious,
explicitly passed expressions, it can be used to model a {constrained
  polymorphism}, and it offers a powerful and disciplined form of
{overloading}.

As a small, but realistic use-case of implicit programming consider a
\emph{polymorphic} sorting function.
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{3}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[3]{}\Varid{sort}\mathbin{:}\forall \alpha\hsforall \hsdot{\circ }{.}\{\mskip1.5mu \alpha\to \alpha\to \Conid{Bool}\mskip1.5mu\}\Rightarrow \Conid{List}\;\alpha\to \Conid{List}\;\alpha{}\<[E]%
\ColumnHook
\end{hscode}\resethooks
Implicit programming offers a convinient way to define such a
function. Sorting cannot be defined as a purely parametric polymorphic
of type \ensuremath{\forall \alpha\hsforall \hsdot{\circ }{.}\Conid{List}\;\alpha\to \Conid{List}\;\alpha}, because it needs to know how to
compare the elements of the list. However \emph{explicitly} passing a
comparison function, can be very tedious: it is likely that for a
given type the sorting function is called with the same comparison
function over and over again. By using an implicit argument for 
passing the comparison function around this problem can be elimated. 

Consider the following program:
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{3}{@{}>{\hspre}l<{\hspost}@{}}%
\column{5}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[3]{}{\bf implicit}\;\{\mskip1.5mu \Varid{cmpInt}\mathbin{:}\Conid{Int}\to \Conid{Int}\to \Conid{Bool}\mskip1.5mu\}\;\mathbf{in}{}\<[E]%
\\
\>[3]{}\hsindent{2}{}\<[5]%
\>[5]{}(\Varid{sort}\;[\mskip1.5mu \mathrm{2},\mathrm{1},\mathrm{3}\mskip1.5mu],\Varid{sort}\;[\mskip1.5mu \mathrm{5},\mathrm{9},\mathrm{3}\mskip1.5mu]){}\<[E]%
\ColumnHook
\end{hscode}\resethooks
The important thing to note is that in this program the two calls of
the sorting function take only one argument: the list to be sorted.
The comparison function used by the sorting function (\ensuremath{\Varid{cmpInt}}) is
\emph{implicitly} passed. It is retrieved automatically from the 
implicit environment in a process called \emph{resolution}. 
In this example, the implicit environment is 
built using the \ensuremath{{\bf implicit}} construct, which is a \emph{scoping}
construct that brings \ensuremath{\Varid{cmpInt}} into the scope of the 
expression \ensuremath{(\Varid{sort}\;[\mskip1.5mu \mathrm{2},\mathrm{1},\mathrm{3}\mskip1.5mu],\Varid{sort}\;[\mskip1.5mu \mathrm{5},\mathrm{9},\mathrm{3}\mskip1.5mu])}.

Scoping and resolution are two essential features of implicit 
programming mechanisms. However, because often implicit 
programming mechanisms are studied in the context of larger 
source language, scoping and resolution do not get the appropriate 
attention and are somehow (artificially) restricted to suit with 
the particular source language.

This paper presents $\ourlang$: a powerful and expressive, yet
minimalistic, calculus for studying the \emph{scoping} and
\emph{resolution} of implicit programming mechanisms.

In the following we will first introduce $\ourlang$ and how its
constructs are useful to model desired functionality in general
implicit programming mechanisms. Then we will expose problems of
existing implicit programming practice with respect to scoping and
resolution, and then summarize our contribution.

\subsection{Modelling Implicit Programming in $\ourlang$}
%% We first introduce, in a general manner, implicit programming by
%% enumerating its essence without being constrained by existing
%% practice. For this purpose we will use our calculus notation. For the
%% readers who are familiar with implicit programming practice, we will
%% sometimes add corresponding examples in notation reminescent of the
%% practice.

%% We then expose problems of existing implicit programming practice 
%% from this general point of view toward implicit programming, and we 
%% summarize our contribution. 

%%\begin{itemize}

%%\item {Implicit programming} fetches values by types and uses types to
%%  infer values. For example the definition of an addition function
%%  that adds one implicit value to an explicit one would be:

%%\begin{verbatim}
%%add : Int => Int -> Int
%%add x = ?Int + x
%%\end{verbatim}

%%To fetch the value of the implicit argument, we use a \emph{query}
%%``$\qask{\tyInt}$''. This query looks up the implicit enviroment for
%%a value associated to the type $Int$.   

%% function $add$ 

\paragraph{Fetching values by types:} $\ourlang$ fetches values by types, not by names.
  For example, the argument for an increment function's can be
  looked up from the implicit environment as follows:
\[
\texttt{inc}\; (\qask{\tyInt}).
\]
The \emph{query} ``$\qask{\tyInt}$'' uses the current implicit
environment to fetch a value of type \tyInt. 

%%Function \texttt{inc} is applied to an argument (we call ``implicit
%%query'') that queries ``$\qask{\tyInt}$'' by mentioning just its
%%type \tyInt.  The int-typed entry in the current implicit
%%environment is looked up  to provide an integer value. 

%%In practice, the implicit query ``$\qask{\tyInt}$'' can even be
%%omitted thanks to type inference. Our calculus makes implicit queries
%%always manifest in text. 

\paragraph{Type-directed rules:} $\ourlang$ constructs values, using
  programmer-defined, type-directed value-resolution rules  (
  similar to functions). Value-resolution rules (rule abstractions) define how
  to compute, from implicit arguments, the values of an intended
  type. For example, a rule that computes a pair of int and bool from
  implicit int and bool values would be:
\[
\qlam{\tyInt, \tyBool}
     {\texttt{(\qask{\tyInt}+1, not\;\qask{\tyBool})}}.
\]
We write the above rule's type as
$\rulety{\tyInt,\tyBool}{\tyInt\times\tyBool}$. 

Hence, where a value of $\tyInt\times\tyBool$ is needed (expressed by 
a query $\qask{(\tyInt\times\tyBool)}$), 
the above rule can be used if int and bool
values are available in the current implicit environment. Under such
environment, the rule returns a pair of the int and bool values after 
respectively incrementing and negating those values. 

Implicit environments are built by rule applications
(analogous to building environments using function applications).
In our notation, rule application is expressed as, for example:
\[
\qapp{\qlam{\tyInt, \tyBool}
      {\texttt{(\qask{\tyInt}+1, not\;\qask{\tyBool})}}
     }{\{\texttt{1},\texttt{true}\}}.
\]
Using a syntactic sugar, which is analogous to the \texttt{let}-expression, the
above application is expressed as:
\[
\qlet{\{\texttt{1},\texttt{true}\}}
     {\texttt{(\qask{\tyInt}+1, not\;\qask{\tyBool})}}
\]
which returns $(2,\Meta{false})$. 

\paragraph{Higher-order rules:} $\ourlang$ supports higher-order
rules. For example, a rule
\[
\qlam{\tyInt,\rulety{\tyInt}{\tyInt\times\tyInt}}{\qask{(\tyInt\times\tyInt)}}
\]
of type
$\rulety{\tyInt,\rulety{\tyInt}{\tyInt\times\tyInt}}{\tyInt\times\tyInt}$ 
computes an integer pair given an integer and a rule to
compute an integer pair from an integer.

Hence, the following example will return $(3, 4)$:
\[
\qlet{\{\texttt{3},\qlam{\tyInt}{\texttt{(\qask{\tyInt},\qask{\tyInt}+1)}}\}}
     {\qask{(\tyInt\times\tyInt)}}.
\]
Resolving (computing a value for) the implicit query
$\qask{(\tyInt\times\tyInt)}$ follows 
a simple inference: the goal is to have a pair of integers, yet the current
environment has no such pair but has an integer $3$ and a rule 
$\qlam{\tyInt}{\texttt{(\qask{\tyInt},\qask{\tyInt}+1)}}$
to compute a pair from an integer. Hence we can apply the pair
construction rule to $3$ to construct the $(3,4)$ pair for the implicit query. 

\paragraph{Polymorphic rules:} $\ourlang$ allows polymorphic rules. For example, rule 
\[
\qLam{\alpha}{\qlam{\alpha}{(\qask{\alpha},\qask{\alpha})}},
\]
whose type is $\forall\alpha.\rulety{\alpha}{\alpha\times\alpha}$, can be
instantiated to multiple rules of monomorphic types
\[
\rulety{\tyInt}{\tyInt\times\tyInt}, 
\rulety{\tyBool}{\tyBool\times\tyBool}, \cdots.
\]
Hence multiple monomorphic queries can be resolved by the same
rule. For example, the following expression returns
$((3,3),(\Meta{true},\Meta{true}))$: 
\[
\begin{array}{l}
\texttt{implicit}\\
\mbox{\ \ \ \ }\{\texttt{3},\;\texttt{true},\;
      \qLam{\alpha}{\qlam{\alpha}{(\qask{\alpha},\qask{\alpha})}}\}\\
\texttt{in}\\
\mbox{\ \ \ \ }
\texttt{(\qask{(\tyInt\times\tyInt)},\qask{(\tyBool\times\tyBool)})}.
\end{array}
\]

\paragraph{Combining higher-order and polymorphic rules:} 
For example, the following rule 
\[
\qlam{\tyInt,\forall\alpha.\rulety{\alpha}{\alpha\times\alpha}}
 {\qask{((\tyInt\times\tyInt)\times(\tyInt\times\tyInt))}}
\]
prescribes how to build a pair of integer pairs, inductively from an
integer value. Begining from an integer value, consecutively applying the 
argument rule of type
\[
\forall\alpha.\rulety{\alpha}{\alpha\times\alpha}
\]
twice: first to an integer, then to its result (an
integer pair) again.

That is, the following expressiong returns $((3,3),(3,3))$:
\[
\begin{array}{l}
\texttt{implicit}\\
\mbox{\ \ \ \ }\{\texttt{3},\;
      \qLam{\alpha}{\qlam{\alpha}{(\qask{\alpha},\qask{\alpha})}}\}\\
\texttt{in}\\
\mbox{\ \ \ \ }
\texttt{\qask{((\tyInt\times\tyInt)\times(\tyInt\times\tyInt))}}.
\end{array}
\]
The $(3,3)$ pair is from applying the rule 
$\qLam{\alpha}{\qlam{\alpha}{(\qask{\alpha},\qask{\alpha})}}$
to $3$, and the final answer $((3,3),(3,3))$ from applying the same
rule to $(3,3)$.

\paragraph{Locally and lexically scoped rules:} Suppose the rule 
\[
\qlam{\tyInt}
 {\qlam{\tyBool, \rulety{\tyBool}{\tyInt}}
       {\qask{\tyInt}}
 }
\]
is applied to an integer and then to a boolean and a rule
of type $\rulety{\tyBool}{\tyInt}$. Resolving the implicit query
$\qask{\tyInt}$ always selects the lexically nearest possible
resolution.

That is, resolution of the implicit query $\qask{\tyInt}$ is not from
fetching the integer value but from applying to the boolean value the
rule that returns an integer from a boolean. Following example thus
returns $2$ not $1$:
\[
\begin{array}{l}
\texttt{implicit}\;\{\texttt{1}\}\;\texttt{in}\\
\mbox{\ \ \ }\texttt{implicit}\;\{\texttt{true},\;
\qlam{\tyBool}{\texttt{if}\;\qask{\tyBool}\;\texttt{then 2}}\}\;\texttt{in}\\
\mbox{\ \ \ \ \ \ }\qask{\tyInt}.
\end{array}
\]

\paragraph{Overlapping rules and coherency:} Two rules overlap if their
  return types intersects, hence they can both be used 
  to resolve the same implicit query. 

  The coherency principle states
  under what conditions the behavior of resolution is consistently
  predictable in the presence of overlapping rules. 
  Without coherency, programming with implicit values is a tricky
  business, fragile and unpredictable. 

  The conherency: the most concrete resolution rule is
  always chosen modulo the lexical scoping. For example, consider the
  following code: 
\[
\begin{array}{l}
\texttt{let}\;\texttt{f}:\forall\beta.\beta\to\beta = \\
\mbox{\ \ \ }\texttt{implicit}\;
  \{\lambda x.x:\forall\alpha.\alpha\to\alpha\}\;\texttt{in}\\
\mbox{\ \ \ \ \ \ }\texttt{implicit}\;
   \{\lambda n.n+1:\tyInt\to\tyInt\}\;\texttt{in}\\
\mbox{\ \ \ \ \ \ \ \ \ }\qask{(\beta\to\beta)}\\
\texttt{in}
\mbox{\ \ \ }\texttt{f} [\tyInt] \texttt{1}\;\cdots\;
             \texttt{f} [\tyBool] \texttt{true}.
\end{array}
\]
The definition of \texttt{f} uses two nested scopes to introduce two
overlapping values in the implicit environment.
According to the consistency principle, resolving the 
implicit query $\qask{\beta\to\beta}$ is determined at \texttt{f}'s
instantiations: the first $f$ must be $\lambda
n.n+1$ and the second $f$ must be $\lambda x.x$. 
%% \end{itemize}

%This \emph{resolution} mechanism to automatically infer
%function arguments based on available type information.  User-supplied
%\emph{rules} determine which values resolution infers. 

\subsection{Problem}
Current implicit programming practice (e.g. Haskell's type classes,
Scala's implicits, C++'s concepts) fails to support 
the above implicit programming features in full combination.

\paragraph{Type classes}
Haskell {type classes}~\cite{adhoc}, which is the
most prominent implicit programming mechanism, explore
only a particular corner of the large design space of implicit
programming~\cite{designspace}, and they have 3 notable limitations:

\begin{itemize}

\item Haskell's resolution rules are global. Hence, there can only be a
single rule for any given
type~\cite{named_instance,overloadingCamarao,implicit_explicit,modular}. No local scoping of rules are available. 
This is an noticeable limitation that already received several proposals for its
fix: rules can be named~\cite{named_instance} or locally
scoped~\cite{overloadingCamarao,implicit_explicit,modular}.
% Kahl and Scheczyk~\cite{named_instance} proposed to address this
%problem with \emph{named instances}, offering the possibility to name
%instances and manually select instances for resolution using these
%names. Others have suggested mechanisms that allowed
%\emph{local scoping} of
%instances~\cite{overloadingCamarao,implicit_explicit,modular}, thus
%offering control over which instances are on scope rather than having
%a single global scope. 
%

\item Haskell type classes are, in some sense, a second class construct
compared to regular types: it is not possible to abstract over a type 
class in Haskell~\cite{restricted}. Yet, the need for first-class type
classes is real in practice~\cite{sybclass, scalageneric}.

\item Finally type classes do not support higher-order rules. As noted by 
Hinze and Peyton Jones~\cite{derivable}, certain Haskell datatypes
like:
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{3}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[3]{}\mathbf{data}\;\Conid{Perfect}\;\Varid{f}\;\alpha\mathrel{=}\Conid{Nil}\mid \Conid{Cons}\;\alpha\;(\Conid{Perfect}\;\Varid{f}\;(\Varid{f}\;\alpha)){}\<[E]%
\ColumnHook
\end{hscode}\resethooks
(a variation of the well-known perfect tree type)
require type class instances such as:
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{3}{@{}>{\hspre}l<{\hspost}@{}}%
\column{5}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[3]{}\mathbf{instance}\;(\forall \beta\hsforall \hsdot{\circ }{.}\Conid{Show}\;\beta\Rightarrow \Conid{Show}\;(\Varid{f}\;\beta),\Conid{Show}\;\alpha)\Rightarrow {}\<[E]%
\\
\>[3]{}\hsindent{2}{}\<[5]%
\>[5]{}\Conid{Show}\;(\Conid{GPerfect}\;\Varid{f}\;\alpha){}\<[E]%
\ColumnHook
\end{hscode}\resethooks
which are not possible to define in Haskell, since Haskell is
restricted to first-order instances (or rules).  This rule is
higher-order because it assumes another rule, \ensuremath{\forall \beta\hsforall \hsdot{\circ }{.}\Conid{Show}\;\beta\Rightarrow \Conid{Show}\;(\Varid{f}\;\beta)}, that itself contains an assumption. Note also that this
assumed rule is polymorphic in \ensuremath{\beta}.  In contrast, as we have seen, in $\ourlang$ such
higher-order rules are allowed:
 \begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{3}{@{}>{\hspre}l<{\hspost}@{}}%
\column{17}{@{}>{\hspre}c<{\hspost}@{}}%
\column{17E}{@{}l@{}}%
\column{21}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[3]{}\forall \Varid{f}\hsforall \;\alpha\hsdot{\circ }{.}\{\mskip1.5mu \forall \beta\hsforall \hsdot{\circ }{.}\{\mskip1.5mu \Conid{Show}\;\beta\mskip1.5mu\}\Rightarrow \Conid{Show}\;(\Varid{f}\;\beta),\Conid{Show}\;\alpha\mskip1.5mu\}{}\<[E]%
\\
\>[3]{}\hsindent{14}{}\<[17]%
\>[17]{}\Rightarrow {}\<[17E]%
\>[21]{}\Conid{Show}\;(\Conid{GPerfect}\;\Varid{f}\;\alpha){}\<[E]%
\ColumnHook
\end{hscode}\resethooks
\end{itemize}

%Finally, type class
%constraints consist, essentially, of first-order rules, %predicates on types,
%but for some applications \emph{higher-order rules} are %predicates} are
%needed~\cite{derivable,scalageneric}.

\paragraph{Scala implicits} The Scala implicits~\cite{implicits}
mechanism provides an interesting alternative implicit programming
design. Unlike type classes it provides locally scoped rules. Moreover
any types can be used as implicit parameters and there's no special 
separate type-class-like interface. Because such interfaces are
modelled with regular types, they can be abstracted over and do 
not suffer from the second class nature of type classes. 

However, implicits only informally described~\cite{implicits,scala}
and some of the design decisions are quite ad-hoc. In particular, 
although Scala allows \emph{nested} local scoping and overlapping rules
\textit{coherence} is not guaranteed, making the use of overlapping
rules quite impredictable. Moreover, Scala does not support
higher-order rules.  

%%The consistency is broken. For the above consistency example, Scala
%%assigns $\lambda x.x$ to both calls to $f$, though $\lambda n.n+1$ is
%%more concrete evidence for $f\;1$.

%differs from Haskell
%type classes in several ways and has its own limitations too.
%In Scala, any value can be made implicit: Scala does not
%segregate type classes and types like Haskell and, as a consequence it
%is possible to abstract over the types representing type
%classes. 
%Secondly, implicit values (which roughly correspond to type
%class instances) are \textit{locally scoped}. 
%%%This allows for the same
%%%type to resolve to different values at different points in the
%%%program.  
%Thirdly, the \textit{scope nesting} prioritizes
%implicits. It enables an important and much desired feature without
%satisfactory solution in the globally-scoped type class approach: how
%to override general rules with ad-hoc cases, known as
%\textit{overlapping rules}.  The Scala solution to overlapping rules is
%  to place the ad-hoc cases in a nested scope, prioritizing them over
%  the general rules in an outer scope. 

%% Finally, it is important to 
%% note that while implicits offer many advantages over type classes, 
%% they have significantly less support for type-inference.


\paragraph{Other mechanisms} Other implicit programming mechanisms sit
in between Haskell type classes and Scala implicits in terms of design
choices. For instance, many proposals for \emph{concepts}, from the
(C++) generic programming community, share with type classes the
segregation between (concept) interfaces and other types, but
emphasize local scoping like Scala implicits. Similarly, the proposal
of Dreyer et al.~\cite{modular} for combining ML-style modules and
type classes distinguishes modules (that model type classes) and other
types, and uses local scoping. Most of these proposals, however, do
not allow overlapping rules nor higher-order ones.

%%\end{itemize}

There is a need to shed more light on the implicit
programming design space from a formal point of view. The existing
literature only addresses features like nested scoping, 
overlapping rules and higher-order predicates independently, but 
it does not provide an account of the combination of these features.
Furthermore the important issue of coherency remains essentially unresolved. 

\subsection{Contribution} 
Our contributions are as follows.
\begin{itemize}
\item We present an \emph{implicit calculus} and a polymorphic type
  system that supports all the
  above mentioned features of implicit  programming: 
our type-safe implicit calculus seamlessly integrates nested scoping,
overlapping rules and higher-order predicates, while at the same time
ensuring coherency in the presence of overlapping rules. 

\item Despite its expressivness, our implicit calculus is a 
minimal system, which makes it ideal for the formal study of
resolution and scoping issues that occur in implicit programming
mechanisms. Furthermore, unlike most existing approaches to implicit
programming, whose semantics are defined by translation, 
our implicit calculus' operational semantics enables a direct
soundness proof and programs can be understood independently of the
type system.  

\item We present a type-preserving translation from our calculus to
  System F, as a way to implement our calculus. 

\item Finally, we present a small, but realistic source language,
  built on top of our calculus, that captures the essence and, in some
  ways, goes beyond the Haskell and Scala implicit programming
  practice. We also sketch the type-directed translation from the
  source to implicit calculus and discuss design decisions related to
  type-inference.

\end{itemize}

%%At the same time, it strives to be
%%a minimal core calculus consisting of only three constructs:
%%1) a query operator, 
%%2) a mechanism for assuming rules in scope, and 
%%3) another mechanism to supply evidence for assumptions.

% simple core calculus that essentially models a query
% language, resembling a simple logic programming language.  It consists of only
% four basic constructs: a query operator, a mechanism for introducing
% facts\tom{rules is a better word, facts in LP are rules without LHS} in scope,
% and another mechanism for binding evidence to facts and eliminating facts. 
% The rule calculus integrates all 4 features discussed by us and, consequently,
% provides a good foundation for studying the issues of scoping and resolution in
% implicit programming mechanisms.

%Technical results

%%We present and compare two semantics for the implicit calculus: a type-directed
%%elaboration semantics and an operational semantics.  While the former is the
%%traditional approach, the latter is the first of its kind for implicit
%%programming: it enables a direct soundness proof and programs can be understood
%%independent of the type system. Moreover, because resolution happens at runtime,
%%a static type system for the operational semantics can accept more programs
%%than for the elaboration semantics, which performs all of resolution statically.

%%In the static type system, we pay particular attention to the different issues
%%that arise with \textit{overlapping rules}, especially with respect to coherency. 
%%Our setting of locally
%%scoped rules and the dynamic resolution in the operational semantic, allows us
%%to formulate alternative solutions for dealing with overlapping rules and
%%avoiding the associated pitfalls.


%%a situation where multiple rules
%%are eligible for resolving an implicit value. Such overlapping rules have shown
%%their use in Haskell and Scala, but
%%the semantic issues are essentially left unaddressed.  


% We present the type system, an operational semantics as well as 
% an elaboration semantics for the polymorphic rule calculus. The 
% operational semantics is proved sound with respect to the type 
% system, and we show that the elaboration semantics is type 
% preserving. Furthermore, both semantics are shown to have 
% the coherency property. Finally, we show that the operational semantics 
% proposed by us is a \emph{conservative extension} of the elaboration 
% semantics, allowing more programs to be accepted, while still preserving 
% coherency. 

% With respect to the operational semantics, it is worth remarking that
% it is the first operational semantics in the literature for an
% implicit programming mechanism. Traditionally, the semantics or
% implementation of implicit programming mechanisms has been through
% elaboration. The large majority of type-class related proposals, Scala
% implicits or proposals for \emph{concepts} in C++ is given a semantics
% in this way.  In this style of semantics there is a source language
% which is translated via a type-directed translation into a core
% language. As a result, soundness can only be proved indirectly, as a
% consequence of the type-preservation of the translation. A consequence 
% of the elaboration semantics is that it tightly couples the dynamic and
% static semantics and it is essentially not possible to understand the
% behavior of programs independently of the type system. Furthermore, 
% it leads to somewhat weaker metatheoretical results~\cite{}.

% Although our operational semantics requires type annotations in
% certain constructs to guide the dynamic execution of programs, 
% it is independent from the static semantics. The operational semantics 
% allows us to prove soundness in a direct style.  Furthermore, it
% offers an alternative to resolution, which is necessarily static 
% in the elaboration semantics. In contrast, our operational semantics 
% allows resolution to happen at run-time, which offers the possibility 
% to accept more programs. Indeed, as we shall see, the operational 
% semantics conservatively extends the elaboration semantics. 

%%We also sketch a simple, but realistic source language that translates to the
%%calculus in a type-directed manner. This source language relinquishes some
%%expressivity to suit type-inference. We discuss the remaining type inference
%%issues and relate them to the literature~\cite{outsidein}.
  


% With respect to related work, the most notable difference of the rule
% calculus is that it focuses on providing a core calculus that directly
% supports features related to implicit programming. Most previous work,
% has typically studied each feature in isolation and has been built
% directly on source languages or core languages that have no built-in
% constructs for supporting implicit programming. For example, with
% respect to local instances, \cite{} proposes an elegant design of type
% classes on top of ML-style modules, which allows instances to be
% selectively activated in a certain local scope. However, none of the
% other 3 features are addressed and the local instances proposed in
% that work cannot be nested (which avoids further issues with respect to
% overlapping instances). 

% \paragraph{Summary}
% The contributions of this paper are:
% \begin{itemize}
% 
% \item \textbf{The rule calculus:} A core calculus aimed at modeling 
% the scoping and resolution features of implicit programming
% mechanisms. 
% 
% \item \textbf{Operational Semantics and dynamic resolution:}
% 
% \item \textbf{Source language and discussion about type-inference:}
% 
% \end{itemize}
% Instead type class interfaces are encoded using
% standard object-oriented interfaces and type class instances correspond to
% implicit objects that implement such interfaces. 

% In comparison to Scala --- which supports a form of local and
% overlapping instances, as well as type classes as types --- the key
% difference is that there is no formalism that models the Scala implicits
% mechanism in the literature. The design of the implicits mechanism is
% only informally described in the Scala reference \cite{}, and in a
% recent paper~\cite{}. More technically, the support for nested local 
% instances is ad-hoc and the current version of Scala does not ensure 
% coherent selection of instances. Furthermore, higher-order predicates 
% are not supported and support for type-inference in Scala is 
% very limited.  
% Notably, Haskell type
% classes assume that instances are globally visible and that there is only one
% possible instance for each type. Furthermore, type classes and types are
% considered distinct entities, the former being predicates (or relations) on the
% latter.

% In particular, the
% following topics have been discussed before in the literature:
% 
% %% * Limitations of type class mechanisms: 
% %%  higher-order predicates, local scoping, first-class type classes, 
% %%  any values can be implicit, overlapping instances. 
% 
% \paragraph{Local scoping} With Haskell type classes instances are
%   globally scoped, which essentially means that there can be only 
%   one instance per type in a program. While there are merits in the
%   choice of global scoping (for example with respect to principal
%   types \cite{}), for certain applications\bruno{mention references,
%     generic programming?} being restricted to a
%   single instance is too limiting and better control over scoping 
%   is desirable. As such, it is not a surprise that several alternative design 
%   proposals include some notion of local scoping
%   \cite{}. \bruno{Want to talk about Scala 
%   here but Scala should first be introduced, come back to this, or see
%   whet. Maybe I can talk about modular type classes later.} 
%    
% \paragraph {Overlapping instances and coherency} Related to scoping is the issue
%   of overlapping instances. Because selection of instances is
%   type-based, there are two important questions related to the
%   selection of instances. Firstly, what should happen if two instances of 
%   the same type are in scope? Secondly, in polymorphic systems like
%   Haskell, what should happen if two instances are in scope but one 
%   is more specific than the other? With global instances the standard 
%   answer to the first question is that programs with two instances of 
%   the same type should be rejected, whereas it is a much debated
%   question of what to do with respect to the second question. With
%   local instances the issue of overlapping instances is even more
%   subtle because for both questions it is debatable what the most 
%   appropriate thing to do is.   
% 
%   Ultimately, the issue of overlapping instances is one of the most
%   controversial in the design of implicit programming
%   mechanisms. While certain implementations of Haskell offer some
%   support for overlapping instances, the semantic foundations of
%   overlapping instances are considered to be quite tricky and there is
%   very little work in that area. Notably a desirable property when
%   dealing with overlapping instances is \emph{coherency}.\bruno{Why 
%   is coherency desirable?}
%   Nevertheless, the experience with
%   Haskell libraries has shown that overlapping instances are useful in
%   practice.\bruno{Again, it may be worth mentioning Scala here,
%     because of the prioritized overlapping implicits, we may also 
%   want to point out that Scala implicits ignore the issue of coherency.}
% 
% \paragraph{Type classes as types} A primary characteristic in the 
% design of Haskell type classes is that regular types (such as
% integers, lists or records) and type classes are segregated. 
% Values of regular types are explicitly passed, and such types 
% can be abstracted through the use of polymorphism. However, 
% with type classes, the evidence (which corresponds to the values) 
% is implicitly passed and type classes cannot be abstracted. 
% While the Haskell design can be justified with the view that 
% type classes as predicates on types, the segregation between 
% type classes and regular types as been shown limiting for certain 
% applications. \bruno{Scala takes a different view}.  
% 
% \paragraph{Higher-order predicates} Finally, in Haskell, constraints 
% can only be first-order predicates. However, in practice the need 
% for higher-order predicates arises. For example, it is well-known
% that instances for datatypes involving parametrization on type constructors, 
% would benefit from higher-order predicates~\cite{}. Also some 
% sophisticated, yet widely used libraries such as the monad transformer 
% library (MTL), are limited in their design partly because of the lack 
% of higher-order predicates. As a result some ad-hoc tricks need to be 
% used to overcome such limitations\bruno{We probably need to
% substantiate this argument. Forward reference to an example in the paper?}. 
% 
% \subsection{The Rule Calculus}
%
% \bruno{What is resolution?}  The main contribution of this paper is
% the \textit{rule caculus}: a calculus aimed at the study of resolution and
% scoping issues that occur in implicit programming mechanisms. From the
% four topics discussed above --- local scoping, overlapping instances,
% type classes as types, and higher-order predicates --- the first 2
% items are related to scoping, whereas the last 2 are related to
% resolution. While, every topic has been discussed before in the
% literature, there are no formalisms capable of providing all the
% features at once (or even some combinations) in the literature. 
% While every feature has shown its use in practice,
% it is not know whether all features can be integrated in a single, coherent
% system. 
% 
% The rule calculus is a simple core calculus that essentially models a query
% language, resembling a simple logic programming language.  It consists of only
% four basic constructs: a query operator, a mechanism for introducing
% facts\tom{rules is a better word, facts in LP are rules without LHS} in scope,
% and another mechanism for binding evidence to facts and eliminating facts. The
% rule calculus integrates all 4 features discussed by us and, consequently,
% provides a good foundation for studying the issues of scoping and resolution in
% implicit programming mechanisms.
% 
% %Technical results
% 
% We present the type system, an operational semantics as well as 
% an elaboration semantics for the polymorphic rule calculus. The 
% operational semantics is proved sound with respect to the type 
% system, and we show that the elaboration semantics is type 
% preserving. Furthermore, both semantics are shown to have 
% the coherency property. Finally, we show that the operational semantics 
% proposed by us is a \emph{conservative extension} of the elaboration 
% semantics, allowing more programs to be accepted, while still preserving 
% coherency. 
% 
% With respect to the operational semantics, it is worth remarking that
% it is the first operational semantics in the literature for an
% implicit programming mechanism. Traditionally, the semantics or
% implementation of implicit programming mechanisms has been through
% elaboration. The large majority of type-class related proposals, Scala
% implicits or proposals for \emph{concepts} in C++ is given a semantics
% in this way.  In this style of semantics there is a source language
% which is translated via a type-directed translation into a core
% language. As a result, soundness can only be proved indirectly, as a
% consequence of the type-preservation of the translation. A consequence 
% of the elaboration semantics is that it tightly couples the dynamic and
% static semantics and it is essentially not possible to understand the
% behavior of programs independently of the type system. Furthermore, 
% it leads to somewhat weaker metatheoretical results~\cite{}.
% 
% Although our operational semantics requires type annotations in
% certain constructs to guide the dynamic execution of programs, 
% it is independent from the static semantics. The operational semantics 
% allows us to prove soundness in a direct style.  Furthermore, it
% offers an alternative to resolution, which is necessarily static 
% in the elaboration semantics. In contrast, our operational semantics 
% allows resolution to happen at run-time, which offers the possibility 
% to accept more programs. Indeed, as we shall see, the operational 
% semantics conservatively extends the elaboration semantics. 
% 
% To illustrate the usefulness of the rule calculus to model realistic
% source languages with implicit programming constructs, we also 
% develop a simple Haskell-like source language which supports 
% the 4 features. This source language can be translated into the rule 
% calculus via a type-directed translation, which is shown to be 
% type-preserving. In the translation the various source language 
% constructs are modeled by combining the rule calculus constructs 
% with the standard constructs of the simply-typed lambda calculus. 
% The resulting language is less expressive than the rule calculus
% itself but, on the other hand, is amenable to type-inference. 
% A discussion about type-inference for this language, as well as
% several examples from the literature are presented.
%   
% With respect to related work, the most notable difference of the rule
% calculus is that it focuses on providing a core calculus that directly
% supports features related to implicit programming. Most previous work,
% has typically studied each feature in isolation and has been built
% directly on source languages or core languages that have no built-in
% constructs for supporting implicit programming. For example, with
% respect to local instances, \cite{} proposes an elegant design of type
% classes on top of ML-style modules, which allows instances to be
% selectively activated in a certain local scope. However, none of the
% other 3 features are addressed and the local instances proposed in
% that work cannot be nested (which avoids further issues with respect to
% overlapping instances). 




% It is not a surprise that alternatives have been proposed. 

%Why is Scala interesting

%%While Scala implicits are implemented and widely used, there is a lot
%%less research exploring the area of the design space covered by Scala.


%%However, important areas of the design space related to scoping and
%%resolution of type class instances remain relatively unexplored.

%%As pointed out by several researchers

%%As an attempt to provide a coherent framework in
%%which many type class extensions can be explained, \cite{} proposed
%%that if type classes are viewed as a particular use mode of ML-modules
%%then many extensions naturally follow for free.

%%Multiple
%%parameter type classes, functional dependencies, associated types 
%%fall in this category.   

%%As noted by several researchers, some of 

%%a lot of the focus of research about type class

%%has been on the ``type classes'' 
%%  (interfaces/ group of methods) part; less has been done on 
%%  scoping and resolution.

%% Following up on the observation that type classes and ML-modules
%% are closely related~\cite{}, \cite{} proposed a module system in which
%% modules can optionally be implicitly passed.

%%* Lots of work on type classes (and also qualified types)
%%  - However, a lot of the focus has been on the ``type classes'' 
%%  (interfaces/ group of methods) part; less has been done on 
%%  scoping and resolution.

%%* While Scala implicits are implemented and widely used, 
%%they have not been formalized.

%%Our solution

%%* The rule calculus. Just 3 constructs that deal with: 
%%  - scoping of implicits (local/lexical/nested scoping/overlapping instances)
%%  - resolution (higher-order predicates/any values of any type) 

%%* Any values of any Types can be implicitly passed (serve as evidence)

%%* Higher-order predicates 

%%* Local Scoping 

%%* First-class type classes

%%* Overlapping instances
%%  + incoherence

%%Operational Semantics

%% * Operational Semantics
%%  - Independent of the static semantics, although types are used to
%%  guide resolution. 

%% * Dynamic Resolution/Static Resolution
%% - coherency   


% \subsection{Old Stuff}
% 
% A recent trend in many programming languages is support for
% \emph{implicit programming}.  \emph{Implicit programming} denotes a
% programming style where some values are automatically inferred by
% using available type information. Implicit programming is 
% useful because it allows implicitly passing many
% values that are tedious to explicitly pass it makes 
% the code more readable 
% 
% . because they simply follow 
% the type structure of another argument, or 
% 
% Haskell type classes~\cite{} are the
% most prominent example of implicit programming. With type classes,
% \emph{type-class implementations} are inferred while performing
% type-inference. For example, in Haskell, the type of the |sort|
% function is as follows:
% 
% > sort :: Ord a => [a] -> [a]
% 
% In this case |Ord a| is a \emph{type-class constraint}. This
% constraint is used to ensure that implementations of comparison
% functions for values of type |a| exist. Such implementations, 
% called type-class instances, are defined by the user 
% 
% In its essence, the type class
% |Ord| is just an interface specifying a number of methods for
% comparing values of some type |a|. 
% 
% The |Ord| type class
% can be implemented for various types such as integers or lists of some
% type |a|. When the |sort| function is called the right implementation
% of |Ord| is selected by the compiler based on the instantiation of the
% type variable |a|. For example, calls like:
% 
% > sort [1,5,3]
% > sort [[1,5],[4,3]]
% 
% describes a particular programming style
% in which certain values used by a program can be \emph{inferred} by
% exploiting type-inference\footnote{This should probably be generalized
% to entail selection based on types, rather than just type-inference}.
% The most prominent example of a mechanism that supports implicit
% programming is given by Haskell type classes. With type classes,
% \emph{type-class dictionaries} (which are a specific kind of records) 
% are inferred while performing type-inference. A canonical
% example is given by a sorting function for lists in Haskell. The type
% of the |sort| function is as follows:
% 
% Implicit programming is to call functions without giving actual
% arguments.
% 
% % Haskell type classes have been widely used and proven to be one
% % effective programming feature. It is originated by the requirement of
% % supporting ad-hoc polymorphism in Hindley-Milner type system. It turns
% % out that we can simulate the things that are considered to only be
% % possible with dependent types with the recent extension of functional
% % dependencies or type families.
% 
% % The key ingredients of Haskell type class are two things: overloading
% % and resolution, whose combination is the essence of what we call {\it
% %   implicit programming}. The use of overloaded entity raises {\it
% %   overloading constraints} which is reflected on the type of
% % expression. For the function with overloading constraints to be used
% % in the later call site, constraints should be {\it resolved} using
% % {\it resolution rules} registered by programmer.
% 
% % Inspired by Haskell type class, many systems with {\it implicit
% %   programming} feature have been proposed.
% 
% % The previous systems have explored the design space of overloading and
% % resolution. \cite{designspace} discusses many design considerations in
% % Haskell type classes. \cite{logic_over,theory_over} studied the
% % resolution. \cite{typeclasses_implicits} studied how Scala-style
% % overloading can support Haskell-style overloading. \cite{without}
% % studied type class-like system in untyped language, Scheme and
% % proposed predicate-based overloading scheme. \cite{modular} proposes
% % an interesting system which harmoniously embeds type class-like
% % feature into ML module system by adding additional usage mode of
% % modules.
% 
% % However, there has not been any work which proposes comprehensive
% % framework on implicit programming. Many systems only supports global
% % scope of resolution rules. Most of them uses
% % static resolution.
% 
% % Especially, the previous systems suffers problem in modular
% % compilation when resolution rules can overlap each
% % other~\cite{designspace}.
% 
% % We propose a general system that is expressive enough to encompass
% % current practices and proposals and solves the intricacy incurred by
% % the overlapping.
% 
% \paragraph{Contributions} Our contributions are as follows.
% 
% \begin{itemize}
% \item We propose a core calculus $\lambda_{\rho}$ which supports the
%   following features of implicit programming:
% 
%   \begin{itemize}
% 
%   \item Flexible implicit values: values of any types can be used as
%     implicit values. This is more general than Haskell type
%     classes~\cite{adhoc} and its extension to named
%     instances~\cite{named_instance, implicit_explicit} where only the
%     dictionaries can be passed implicitly.
% 
%     % Note that in
%     % Haskell type classes~\cite{adhoc} and its extension to named
%     % instances~\cite{named_instance, implicit_explicit}, only
%     % dictionaries can be passed to functions implicitly. This is
%     % generalized in ~\cite{modular} such that modules are used as
%     % implicit values, but this is still limited because modules are not
%     % first-class objects in their system.
% 
%   \item Lexical scoping: an implicit value has lexical scope where it
%     is used for resolution. Lexical scopes of implicit values can be
%     arbitrarily nested. Again, this is more general than the systems
%     with only global scope~\cite{adhoc, theory_over, snd_over,
%       logic_over}.
% 
%   \item Overlapping instances: two implicit instances can overlap each
%     other in the same implicit scope unless they make
%     ambiguity. Overlapping instances is regarded as a useful feature
%     but has not yet been handled properly~\cite{designspace}.
%     Especially, the combination of overlapping instances and lexical
%     scoping has not yet been discussed.
% 
%     % \item First-class instances: implicit instances can be freely
%     %   created, passed and registered to implicit scope at run
%     %   time. First-class instances are necessary for generic
%     %   programming~\cite{syb, sybclass}, so they have been partially
%     %   supported by Glasgow Haskell Compiler~\cite{ghc}. However, there
%     %   is no system that fully supports this.
% 
%     % \item High-order implicit constraints: as an additional benefit of
%     %   flexible implicit values, we can use types with higher-order
%     %   implicit constraints. 
% 
%   \end{itemize}
% 
%   These features have not yet been combined in any single system
%   proposed in the literature.
%   
% \item For our language, we provide two alternatives for resolving
%   implicit constraints; dynamic resolution, which always picks the
%   most specific instance for the given constraint but is not modular,
%   and static resolution, which is modular but fails to pick the most
%   specific one when there are overlapping instances. We explain in
%   detail about for which set of programs both resolution coincide and
%   for which they do not.
% 
% \item Based on our core calculus, we make a simple language that
%   supports all the features of core calculus with some restrictions
%   and still enjoys the benefits of type inference. There has been no
%   system that has all these features with type inference.
% 
% % \item High-order implicit constraints:
% 
% \end{itemize}

% \paragraph{Organization} Section \ref{sec:overview} is an overview of
% our calculus $\ourlang$ and shows how our calculus supports various
% features of implicit programming using examples. Section
% \ref{sec:notation} defines notations to be used in the rest of this
% paper. Section \ref{sec:calculus} presents the formal system of
% $\ourlang$; operational semantics, polymorphic type system and
% type-directed translation are explained. Section \ref{sec:resolution}
% shows a detailed study on resolution in our system. Section
% \ref{sec:example} gives an example Haskell-like programming language
% as an instance of our general framework. Section \ref{sec:discussion}
% discusses some issues. Section \ref{sec:related} presents our
% exhaustive study on the previous work and comparison results. Section
% \ref{sec:conclusion} concludes.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../Main"
%%% End: 


==> src/Over.tex <==
%% ODER: format ==         = "\mathrel{==}"
%% ODER: format /=         = "\neq "
%
%
\makeatletter
\@ifundefined{lhs2tex.lhs2tex.sty.read}%
  {\@namedef{lhs2tex.lhs2tex.sty.read}{}%
   \newcommand\SkipToFmtEnd{}%
   \newcommand\EndFmtInput{}%
   \long\def\SkipToFmtEnd#1\EndFmtInput{}%
  }\SkipToFmtEnd

\newcommand\ReadOnlyOnce[1]{\@ifundefined{#1}{\@namedef{#1}{}}\SkipToFmtEnd}
\usepackage{amstext}
\usepackage{amssymb}
\usepackage{stmaryrd}
\DeclareFontFamily{OT1}{cmtex}{}
\DeclareFontShape{OT1}{cmtex}{m}{n}
  {<5><6><7><8>cmtex8
   <9>cmtex9
   <10><10.95><12><14.4><17.28><20.74><24.88>cmtex10}{}
\DeclareFontShape{OT1}{cmtex}{m}{it}
  {<-> ssub * cmtt/m/it}{}
\newcommand{\texfamily}{\fontfamily{cmtex}\selectfont}
\DeclareFontShape{OT1}{cmtt}{bx}{n}
  {<5><6><7><8>cmtt8
   <9>cmbtt9
   <10><10.95><12><14.4><17.28><20.74><24.88>cmbtt10}{}
\DeclareFontShape{OT1}{cmtex}{bx}{n}
  {<-> ssub * cmtt/bx/n}{}
\newcommand{\tex}[1]{\text{\texfamily#1}}	% NEU

\newcommand{\Sp}{\hskip.33334em\relax}


\newcommand{\Conid}[1]{\mathit{#1}}
\newcommand{\Varid}[1]{\mathit{#1}}
\newcommand{\anonymous}{\kern0.06em \vbox{\hrule\@width.5em}}
\newcommand{\plus}{\mathbin{+\!\!\!+}}
\newcommand{\bind}{\mathbin{>\!\!\!>\mkern-6.7mu=}}
\newcommand{\rbind}{\mathbin{=\mkern-6.7mu<\!\!\!<}}% suggested by Neil Mitchell
\newcommand{\sequ}{\mathbin{>\!\!\!>}}
\renewcommand{\leq}{\leqslant}
\renewcommand{\geq}{\geqslant}
\usepackage{polytable}

%mathindent has to be defined
\@ifundefined{mathindent}%
  {\newdimen\mathindent\mathindent\leftmargini}%
  {}%

\def\resethooks{%
  \global\let\SaveRestoreHook\empty
  \global\let\ColumnHook\empty}
\newcommand*{\savecolumns}[1][default]%
  {\g@addto@macro\SaveRestoreHook{\savecolumns[#1]}}
\newcommand*{\restorecolumns}[1][default]%
  {\g@addto@macro\SaveRestoreHook{\restorecolumns[#1]}}
\newcommand*{\aligncolumn}[2]%
  {\g@addto@macro\ColumnHook{\column{#1}{#2}}}

\resethooks

\newcommand{\onelinecommentchars}{\quad-{}- }
\newcommand{\commentbeginchars}{\enskip\{-}
\newcommand{\commentendchars}{-\}\enskip}

\newcommand{\visiblecomments}{%
  \let\onelinecomment=\onelinecommentchars
  \let\commentbegin=\commentbeginchars
  \let\commentend=\commentendchars}

\newcommand{\invisiblecomments}{%
  \let\onelinecomment=\empty
  \let\commentbegin=\empty
  \let\commentend=\empty}

\visiblecomments

\newlength{\blanklineskip}
\setlength{\blanklineskip}{0.66084ex}

\newcommand{\hsindent}[1]{\quad}% default is fixed indentation
\let\hspre\empty
\let\hspost\empty
\newcommand{\NB}{\textbf{NB}}
\newcommand{\Todo}[1]{$\langle$\textbf{To do:}~#1$\rangle$}

\EndFmtInput
\makeatother
%

\section{Overview} %%of Rule Calculus $\ourlang$}
\label{sec:overview}

In this section, we motivate and give an overview of the rule calculus and the
source language described in Section~\cite{}. 

%%The rule calculus is
%%presented as a simple logic programming language of Horn clauses
%%and the relation to existing implicit programming mechanisms is
%%discussed. Then it is shown how a source language built on top 
%%of the rule calculus can model 

\subsection{Rule Calculus $\ourlang$ Syntax}

\begin{figure}

\begin{center}
  
  \[ \begin{array}{llrl}
    \text{Types} & \type  & ::=  & \alpha \mid \rulet \\
    \text{Rule Types} & \rulet  & ::= & 
    \rulesch{\alpha}{\rulesetvar}{\type} \\
    \text{Context} & \rulesetvar  & ::= & \bar{\rulet} \\
    \text{Expressions} & e & ::=  & 
    ?\rulet \mid 
    \ruleabs{\rulet}{e} \mid
    e[\overline{\type}] \mid
    \ruleapp{e}{\rulesetexp} \\
  \end{array} \]
\end{center}

\caption{Rule calculus syntax}

\end{figure}

\subsection{Rules and Rule Types}

The key notion of the rule calculus is that of a rule and its
corresponding rule type. Rule types are 

Relation to type classes; well-known relation between 
type classes and logic programming.

\paragraph{Horn clauses as rule types}

\Ex{
  1) \quad \{\} \To \tyint \\
  2) \quad \{\tybool\} \To \tyint \\
  3) \quad \{a \to a \to \tybool \} \To [a] \to [a] \to [a]  \\
  4) \quad \{\Eq~a\} \To [a] \to [a] \to [a] \\
  5) \quad \{\Eq~a, \Eq~b\} \To \Eq~(a,b)   
}

\paragraph{Polymorphic and higher-order rules}

\subsection{Resolution and Queries}

\paragraph{Higher-order queries}

\subsection{Scoping}

\paragraph{Local Scoping}

\paragraph{Nested Scoping}

\paragraph{Overlapping}

\subsection{Source Language and Type-Inference}

present $\ourlang$ and its core features using
some examples. The formal system of the calculus is presented in
Section~\ref{sec:calculus}. In the rest of this section, we assume
that the calculus is conservatively extended to have constructs of
$\lambda$-calculus and several types.

$\ourlang$ is a simple logic programming language of Horn clauses. We
can compose Horn clauses and resolve a clause under the given set of
clauses. Consider the following example:
\\
\Ex{
  \relation{f}{\myset{\tyint} \To \tyint} \\
  f = \ruleabs{(\myset{\tyint} \To \tyint)}{(?\tyint + 1)} \\
}
\\
In the example, $f$ is a {\it rule} whose type corresponds to Horn
clause $\tyint \To \tyint$. The clause, which we call {\it rule type},
means that $f$ will give us an integer value if there is an integer
clause in the assumptions. We call the current set of assumptions as
{\it rule environment}. In the body, the rule tries to resolve query
$?\tyint$ which essentially asks whether the rule type $\tyint$ can be
deduced from the given assumptions. Since $f$ assumes that there must
be a rule type $\tyint$, the query can be resolved. If we apply this
rule to a rule of type $\tyint$, we can get the final value like this:
\\
\Ex{ \ruleapp{f}{\myset{\relation{1}{\tyint}}} }
\\
This program will give us 2 as a result.

The rule type can be polymorphic in $\ourlang$. Consider the following
example:
\\
\Ex{
  \relation{g}{\myset{\forall \alpha. \alpha \to \alpha} \To 
    \tyint \to \tyint} \\
  g = \ruleabs{(\myset{\forall \alpha. \alpha \to \alpha} \To 
    \tyint \to \tyint)}{(?\tyint \to \tyint)} \\
}
\\
The query $?\tyint \to \tyint$ can be resolved by instantiating the
assumption $\forall \alpha. \alpha \to \alpha$ for the $\tyint$
type. 

In the rest of the section, we explain the key features that
differentiate our calculus from the others. Note that some of these
features have already existed in the previous systems but none of them
provides the combination of all.

\subsection{Flexible Implicit Values}
\label{subsec:flexible}

We allow arbitrary types in rule types. This is different from type
class-like systems. The type class-like systems can be modeled as
simple logic language with Horn clauses of predicates on
types. Rather, our system is closer to Scala implicits~\cite{scala}.

Using arbitrary types for the assumptions has more flexibility than
using only predicates on types. Because of this limitation, some
Haskell programs try to encode natural number using type-level Church
numeral to do the very same thing like this:

\[  
\begin{array}{l}
  \relation{f}{\myset{\tyint} \To \tyint} \\ 
  f = \ruleabs{(\myset{\tyint} \To \tyint)}{(?\tyint + 1)}
\end{array}
\]
\[  
\begin{array}{l}
  \ruleapp{f}{\myset{\relation{\ruleabs{(\varnothing \To
          \tyint)}{1}}{\varnothing \To \tyint}}}
\end{array}
\]

\subsection{Lexical Scoping}
\label{subsec:lexical}

We support lexical scoping of rule environments. Consider the
following example:
\\
\[  
\begin{array}{l}
  \ruleapp
  {\ruleapp{f}{\myset{\relation{2}{\tyint}}}}
  {\myset{\relation{1}{\tyint}}}
\end{array}
\]
\\
The rule $f$ is now put under two environments. 

Under the nesting, we choose the closest one from the given rule.

\subsection{Overlapping}
\label{subsec:overlapping}

We allow overlapping of rules. 

\[
\begin{array}{l}
  \relation{f}{\forall \alpha. \alpha \to \alpha} \\
  f = 
  \ruleapp
  {(\ruleabs
    {(\forall \alpha.
      \myset{\forall \beta. \beta \to \beta, \tyint \to \tyint}
      \To \alpha \to \alpha)
    }
    {(?\alpha \to \alpha)})\\\quad\quad}
  {\myset{
      \relation{\lambda x. x + 1}{\tyint \to \tyint},
      \relation{\lambda x. x}{\forall \gamma. \gamma \to \gamma}
    }}
\end{array}
\]

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../Main"
%%% End: 


==> src/Rel.tex <==
%% ODER: format ==         = "\mathrel{==}"
%% ODER: format /=         = "\neq "
%
%
\makeatletter
\@ifundefined{lhs2tex.lhs2tex.sty.read}%
  {\@namedef{lhs2tex.lhs2tex.sty.read}{}%
   \newcommand\SkipToFmtEnd{}%
   \newcommand\EndFmtInput{}%
   \long\def\SkipToFmtEnd#1\EndFmtInput{}%
  }\SkipToFmtEnd

\newcommand\ReadOnlyOnce[1]{\@ifundefined{#1}{\@namedef{#1}{}}\SkipToFmtEnd}
\usepackage{amstext}
\usepackage{amssymb}
\usepackage{stmaryrd}
\DeclareFontFamily{OT1}{cmtex}{}
\DeclareFontShape{OT1}{cmtex}{m}{n}
  {<5><6><7><8>cmtex8
   <9>cmtex9
   <10><10.95><12><14.4><17.28><20.74><24.88>cmtex10}{}
\DeclareFontShape{OT1}{cmtex}{m}{it}
  {<-> ssub * cmtt/m/it}{}
\newcommand{\texfamily}{\fontfamily{cmtex}\selectfont}
\DeclareFontShape{OT1}{cmtt}{bx}{n}
  {<5><6><7><8>cmtt8
   <9>cmbtt9
   <10><10.95><12><14.4><17.28><20.74><24.88>cmbtt10}{}
\DeclareFontShape{OT1}{cmtex}{bx}{n}
  {<-> ssub * cmtt/bx/n}{}
\newcommand{\tex}[1]{\text{\texfamily#1}}	% NEU

\newcommand{\Sp}{\hskip.33334em\relax}


\newcommand{\Conid}[1]{\mathit{#1}}
\newcommand{\Varid}[1]{\mathit{#1}}
\newcommand{\anonymous}{\kern0.06em \vbox{\hrule\@width.5em}}
\newcommand{\plus}{\mathbin{+\!\!\!+}}
\newcommand{\bind}{\mathbin{>\!\!\!>\mkern-6.7mu=}}
\newcommand{\rbind}{\mathbin{=\mkern-6.7mu<\!\!\!<}}% suggested by Neil Mitchell
\newcommand{\sequ}{\mathbin{>\!\!\!>}}
\renewcommand{\leq}{\leqslant}
\renewcommand{\geq}{\geqslant}
\usepackage{polytable}

%mathindent has to be defined
\@ifundefined{mathindent}%
  {\newdimen\mathindent\mathindent\leftmargini}%
  {}%

\def\resethooks{%
  \global\let\SaveRestoreHook\empty
  \global\let\ColumnHook\empty}
\newcommand*{\savecolumns}[1][default]%
  {\g@addto@macro\SaveRestoreHook{\savecolumns[#1]}}
\newcommand*{\restorecolumns}[1][default]%
  {\g@addto@macro\SaveRestoreHook{\restorecolumns[#1]}}
\newcommand*{\aligncolumn}[2]%
  {\g@addto@macro\ColumnHook{\column{#1}{#2}}}

\resethooks

\newcommand{\onelinecommentchars}{\quad-{}- }
\newcommand{\commentbeginchars}{\enskip\{-}
\newcommand{\commentendchars}{-\}\enskip}

\newcommand{\visiblecomments}{%
  \let\onelinecomment=\onelinecommentchars
  \let\commentbegin=\commentbeginchars
  \let\commentend=\commentendchars}

\newcommand{\invisiblecomments}{%
  \let\onelinecomment=\empty
  \let\commentbegin=\empty
  \let\commentend=\empty}

\visiblecomments

\newlength{\blanklineskip}
\setlength{\blanklineskip}{0.66084ex}

\newcommand{\hsindent}[1]{\quad}% default is fixed indentation
\let\hspre\empty
\let\hspost\empty
\newcommand{\NB}{\textbf{NB}}
\newcommand{\Todo}[1]{$\langle$\textbf{To do:}~#1$\rangle$}

\EndFmtInput
\makeatother
%
%%format in="\Varid{in}"

\section{Related Work}
\label{sec:related}

%%This section discusses related work.
%
%In Section~\ref{subsec:problem} we have already discussed the main
%distinguishing factors between our work and Haskell's type classes, Scala's 
%implicits, and some other systems. In what follows, 

We first summarize how our work is in general different from existing
work and then compare in more detail our work with existing work with
respect to scoping, overlapping, coherence, semantics and resolution. 
%
%% \subsection{Scoping and Resolution}

Our work distinguishes itself from previous work in several respects. 
We capture the key features of 
IP in a minimalist and core calculus $\ourlang$. The calculus
shows a seamless integration of a number of
IP features --- local and nested scoping;
higher-order rules and queries; and overlapping rules --- that have
only been studied in isolation before. Furthermore, the calculus'
minimalistic and core nature makes it an ideal platform for a study of
key issues in IP such as scoping and resolution. In contrast,
most existing IP mechanisms have been implemented or
studied as part of a larger source language, hence some artificial restrictions
that are imposed by the intricacies of the source language, which makes the
study of issues such as scoping and resolution hard. 
Finally, thanks to the calculus we can understand and address the
problem of ensuring coherence in the presence of overlapping rules and
nested scoping. 

%%\subsection{Design choices}
%%The design space of implicit programming mechanisms is quite big.
%%Various implicit programming mechanisms considerably differ in their
%%design. 


%
%
%%if False
%
%The fact that $\ourlang$ does not provide a special type of ``type
%class'' interface, does not preclude the definition of source
%languages which have such interfaces. In fact, $\ourlang$ is a
%good target language for a language with type classes, or some other
%form of interfaces (such as modules or object-oriented classes).  The
%main challenges of provide a source language with type classes are
%type-inference and subclassing. In Section~\ref{} we have already
%discussed how the issue of type-inference can be overcome for a simple
%language with records. In a source language with type classes, type
%inference could be dealt pretty much in the same way. Furthermore,
%subclassing is not hard to translate to $\ourlang$~\bruno{Tom, say
%  more about this?}. 
%
%Another advantage of allowing any types in resolution is that
%higher-order predicates come essentially for free. Since we can query
%any types and have any types in the implicit environment, supporting
%higher-order predicates amounts to allowing polymorphic rule types to
%be queried.
% 
%One way in which our calculus is closer to type classes is that 
%implicit arguments are sets rather than lists (as in Scala). 
%
%> let f : {Int} => 
%
%> let f   
%
%Compared with type classes, this
%design is, in some sense, more primitive as it  
%
%and it has some drawbacks in terms of usability. Namely and refinement
%(subclass) relations between class interfaces allow programmers to
%express certain constraints more conveniently. Scala implicits are
%expressive enough to encode the same essential programming patterns
%expressible with types classes~\cite{implicits}, but the encoding can
%make the programming-style more low level than type classes due to
%type-inference limitations, and the need to encode subclassing.
%
%Usability concerns are not so important in a core calculus, where
%expressiveness and simplicity of the design are more relevant. 
%
%By allowing any types to be involved in the resolution process, 
%the implicit calculus  
%
%%endif
%
%%%Another important different to previous work is the minimalistic 
%%%and core nature of our calculu
%
%%if False
%
%% Scoring:
%\newcommand{\scri}[1]{\quad\small #1}% sub-criterion
%\newcommand{\scgood}{\CIRCLE}% good
%\newcommand{\scsuf}{\LEFTcircle}% sufficient
%\newcommand{\scbad}{\Circle}% bad
%
%\newcommand{\latexhline}{\hline}
%
%\begin{figure*}
%\tabcolsep\arraycolsep
%\def\tallstrut{\vrule width0pt height 2.5ex}
%\def\deepstrut{\vrule width0pt height 0pt depth 1.5ex}
%\begin{center}
%\begin{tabular}{l||c||cccc||ccc||cc||c}
%& \multicolumn{1}{c}{\textit{Scala}} & \multicolumn{4}{c}{\textit{Type Classes}} & \multicolumn{3}{c}{\textit{Overloading}} &  \multicolumn{2}{c}{\textit{Others}} & \multicolumn{1}{c}{\textit{$\ourlang$}} \\
%                                          &                 & Wad89       & \textit{Kah01}     & \textit{Dij05}  & \textit{Dre07}    & \textit{O} & \textit{CT} & \textit{Sul05} & \textit{Lew00} & \textit{Gar05} & 
%\deepstrut \\
%\latexhline % ---------------------------------------------------------------
%\tallstrut
%Design choices:                                 &                 &             &                    &                 &                   &                  &                &                &                &           & \\
%\scri{Overloaded Entities}                & Type            & Name        &  Name              & Name            & Name                 & Name             & Name           & Name           & Name              & Name        & Type \\
%\scri{Constraint Semantics}               & [T]             & \{C\}       &  [C$\mid$\{C\}]        & [C]           & \{M\}             & \{N$\times$T\}   & \{N$\times$T\} & \{N$\times$T\} & \{N$\mapsto$T\}& -        & \{T\}   \\
%% \scri{First-class Types}                  & \scgood         & \scbad      &  \scbad            & \scbad          & \scbad            & \scgood          & \scgood        & \scgood        & \scgood        & \scbad  & \scgood \\
%\scri{Implicit Values}                    & \scgood         & \scbad      &  \scbad            & \scbad          & \scbad            & \scgood          & \scgood        & \scgood        & \scgood        & \scbad  & \scgood \\
%\scri{Any Values}                         & \scgood         & \scgood     &  \scgood                 & \scgood               & \scgood           & \scbad           & \scgood        & \scgood        & \scgood              & \scbad        & \scgood \\
%\scri{Overloaded Results}                 & \scgood         & \scgood     &  \scgood                 & \scgood               & \scgood           & \scbad           & \scgood        & \scgood        & -              & \scbad   & \scgood \\
%Resolution:                                    &                 &             &                    &                 &                   &                  &                &                &                &           & \\
%\scri{Recursive Resolution}               & \scgood         & \scgood     &  \scgood           & \scgood         & \scgood           & \scgood         & \scgood              & \scgood       & \scbad         & \scgood        & \scgood \\
%\scri{Higher-order Predicates}               & \scbad             & \scbad       &  \scbad        & \scbad           & \scbad             & \scbad   & \scbad & \scbad & \scbad & \scbad        & \scgood   \\
%% \scri{Contextual Overloading}             & \scbad          & \scbad      &  \scbad            & \scbad          & \scbad            & \scbad           & \scgood        & \scbad         & -         & -        & \scbad \\
%% \scri{Polymorphic Type}                   & \scgood         & \scgood     &  \scgood                 & \scgood               & \scgood           & \scgood          & \scgood         & \scgood        & \scbad              & -     & \scgood \\
%Scoping:                                    &                 &             &                    &                 &                   &                  &                &                &                &           & \\
%\scri{Lexical Scoping}                    & \scgood         & \scbad      &  \scbad            & \scgood         & \scgood           & \scbad           & \scgood        & \scbad         & \scgood        & \scgood  & \scgood \\
%\scri{Nested Scoping}                     & \scsuf          & \scbad      &  \scbad            & \scgood         & \scbad           & \scbad           & \scgood         & \scbad         & \scgood        & \scgood  & \scgood \\
%\scri{Overlapping}                       & -         & -      &  -            & -         & -           & -           & -         & -         & -        & -  & - \\
%Semantics and Coherence:                                    &                 &             &                    &                 &                   &                  &                &                &                &           & \\
%\scri{Coherence}                         & -         & -      &  -            & -         & -           & -           & -         & -         & -        & -  & - \\
%\scri{Resolution Time}                & -         & -      &  -            & -         & -           & -           & -         & -         & -        & -  & - \\
%\scri{Semantics}                          & -               & E           & -                  & E               & E                 & E/D              & -              & E              & E/A            & -        & O/E     \\     
%Source Language:                                    &                 &             &                    &                 &                   &                  &                &                &                &           & \\
%\scri{Overriding}                         & \scgood         & \scbad      &  \scgood           & \scgood         & \scbad           & \scbad           & \scsuf         & \scbad         & \scgood        & \scbad & \scsuf       \\
%\scri{Constraint Inference}               & \scbad          & \scgood     &  \scgood           & \scgood         & \scgood                 & \scgood          & \scgood        & \scgood        & \scgood        & -        & \scgood \\
%\scri{Context Reduction}                  & \scbad          & \scgood     &  \scbad           & \scgood         & \scgood           & \scbad         & \scgood              & \scgood       & \scbad         & -        & \scgood \\
%\scri{Late Binding}                       & \scgood         & \scbad      &  \scgood           & \scgood               & \scgood                 & \scbad           & \scbad         & \scbad         & \scbad         & \scgood  & \scgood \\
%%%Others:                                    &                 &             &                    &                 &                   &                  &                &                &                &           & \\
%%%\scri{Flexible Type                     & -               & \scbad      &  \scbad                 & \scbad               & \scbad                 & \scgood          & \scsuf             & \scbad         & -              & -        & - \\
%%%\latexhline % ---------------------------------------------------------------
%%%Formalization:                            & \scbad          & \scgood     & \scsuf             & \scsuf          & \scgood           & \scgood          & \scsuf         & \scgood        & \scgood        & \scbad   & \scgood \\
%%%\scri{Metatheory Results}                 & -               & \scgood     & \scsuf             & \scbad          & \scgood           & \scgood          & \scsuf         & \scgood        & \scgood        & -        & \scgood \\     
%%%\scri{Machine Checked}                    & -               & \scbad      & \scbad             & \scbad          & \scbad            & \scbad           & \scbad         & \scbad         & \scbad         & -        & \scgood \\     
%\deepstrut \\
%\end{tabular}
%\end{center}
%
%\begin{tabular}{c||c}
%Abbreviations used in the Constraint semantics row & Abbreviations used in the Semantics row \\
%\begin{tabular}{c||l}
%T & Type\\
%C & Type Class\\
%M & Module\\
%N & Name\\
%\end{tabular}&
%\begin{tabular}{c||l}
%E & Elaboration Semantics\\
%A & Axiomatic Semantics\\
%D & Denotational Semantics\\
%O & Operational Semantics\\
%\end{tabular}\\
%\end{tabular}
%
%\caption{The design space of mechanisms related to implicit
%  programming.\bruno{Need to adapt the figure to fit with the
%    structure of the overview.}}
%\label{fig:evaluation}
%\end{figure*}
%
%To aid with the comparison to related work we summarize the features  
%available in various systems in Figure~\ref{}, and compare it with our 
%own work. In the table, only features related to scoping and
%resolution are discussed. 
%
%%endif

\paragraph{Scoping, Overlapping, and Coherence}
%Several works have discussed scoping mechanisms for IP. 
Our work allows nested scoping with overlapping rules
while guaranteeing coherence. Regarding these issues, previous
approaches can be divided into two types. The first type of
approaches allow local scoping but forbid nested scoping and, as
such, avoid the issue of guaranteeing coherence in the presence of
overlapping. Modular type
classes~\cite{modular} and System $F_{G}$~\cite{fg} are examples of
such approaches. The second type of approaches allow nested scoping,
but do not guarantee coherence. Most prominently, Scala falls in this
category, but there are several other proposals that also follow such
approach~\cite{systemct,implicit_explicit,instanceargs}.

The GHC Haskell compiler supports overlapping instances~\cite{designspace},
that live in the same global scope. Our calculus generalizes this idea to
local scoping. The problem with GHC's scope is that deciding coherence requires
global information. This is at odds with modular compilation. As GHC prefers
the latter, it does not perform a full coherence check and thus cannot
guarantee coherence across modules.

Our calculus is different from \emph{instance chains}~\cite{chain}
too. With instance chains the programmer imposes an
order on a set of overlapping type class instances. All instance
chains for a type class have global scope and are expected not to
overlap. This makes the scope of overlapping closed within a chain,
which is one way to ensure the coherence under the presence of
overlap. In our calculus, we make our local scope closed,
thus overlap only happens within one nested scope.

Lastly, Jones~\cite{coherence_qual} discussed about the coherence of
qualified type system in his work on qualified types. In their
definition, the translation semantics is coherent if the given
system of predicates guarantees the uniqueness of evidence. Their coherence
provides a general framework for Haskell-like systems, but it leaves
out the details about how to coherently generate the evidence, which
is non-trivial with overlapping instances.

\paragraph{Semantics}
%\bruno{This paragraph needs to be rewritten!}

Our calculus' dynamic semantics is defined in a big-step operational
semantics. This contrasts with the majority studies of IP mechanisms.
The majority have a semantics based on translation,
in which the queries are resolved statically. Several
researchers~\cite{tchaskell,snd_over} have pointed out that an
translation semantics is a weakness of those systems: the static and
dynamic semantics cannot be understood independently, and there is no
semantic soundness result. Though Thatte's work~\cite{semantics_typeclass},
which is one exception, translates a program with type classes
into one of an ML-like calculus with typecase and fixpoint
operator, the resolution in the translated program is done
dynamically. Still the work suffers from having no direct soundness
result with respect to the dynamic semantics.

There is a few other works that provide a dynamic semantics for IP,
but they have some restrictions that our calculus' operational
semantics does not. Notable such works are by Odersky et
al. \cite{snd_over} and Kaes \cite{kaes}. Their systems provide
both translation and denotational semantics for their overloading
mechanisms. % As as far as we know, $\ourlang$ is
% the third system provides dynamic semantics as a foundation for type
% system and translation. 
% Kaes's work \cite{kaes} is one of the earliest work in the type class
% field. 
However, Kaes's system does not 
support overlapping, local scoping and polymorphic instances. 
Odersky et al.'s system, cannot make instances that are polymorphic
on the return type. Besides, their dynamic semantics require runtime
type information to resolve overloaded instances. Our operational semantics, on
the contrary, has none of these restrictions and does not need to
check the type of value at runtime. 

%\bruno{Shouldn't
%  the point here be the fact that our operational semantics does *not* dependent 
%on the static semantics, whereas their dynamic semantics *depends* on
%the static semantics.}

%However the dynamic semantics is still coupled with the
%static semantics. (some amount of type-checking is needed at
%run-rime). \bruno{Others?}

%The implicit calculus distinguishes also does have an operational semantics. In
%this operational semantics types cannot be erased. However, the operational
%semantics itself is independent of the type system and we can prove semantic
%soundness.

%Our operational semantics has an additional advantage: it features run-time
%resolution. In the presence of overlapping instances, this allows us to accept
%more programs than the elaboration semantics.
%\wt{This is not true any more}

%\bruno{Say more about related work``typecase'' stuff; Kaes?}
%
%\bruno{Do we want to go into details? Probably not, but if we want we
%  can add the text below.}

%- - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
\paragraph{Resolution}
Resolution in $\ourlang$ is significantly more expressive than in
other systems. Notably resolution supports higher-order rule types and
queries, as well as queries for polymorphic types. A closely related
design is that of higher-order predicates by Hinze and Peyton
Jones~\cite{derivable}. However, similar extensions have not been
adopted by any other IP systems.

As such, the interaction with other features is first studied by our work.
Notably, Hinze and Peyton Jones propose the more expressive resolution rule,
but do not consider our main reason for adopting a simpler definition: its
impact on guaranteeing coherence in the presence of overlap (as well as
guaranteeing termination).

As Hinze and Peyton Jones show, higher-order predicates are specially important
when dealing with types that involve type constructor polymorphism. In order to
simplify presentation, our formalization of the implicit calculus does not
include type constructor polymorphism. However, such an extension is
straightforward, as our implementation shows.

\paragraph{``Type class'' interfaces}
$\ourlang$ focuses on scoping and resolution, which contrasts with a
lot of recent work on IP mechanisms, where the focus
has been on increasingly more powerful ``type class'' interfaces. For
instance, \emph{functional dependencies}~\cite{fundeps},
\emph{associated types}~\cite{assoctypes,assoctypes2} and \emph{type
  families}~\cite{typefunc} are all examples of this trend. This line
of work is orthogonal to ours. In essence, although $\ourlang$ does
not provide a special type of ``type class'' interface natively, this
does not preclude the definition of source languages which have such
interfaces. The idea is that such interfaces can be added as
extensions, very much in the same way that we added records in our
source language in Section~\ref{sec:example}. The design of Scala implicits,
modular type classes and instance arguments~\cite{instanceargs} in Adga shows that,
when a good notion of interfaces exists in the base language, the
addition of an IP mechanism makes many advanced
features such as associated types fall out essentially for free.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../Main"
%%% End: 


==> src/Resolution.tex <==

\section{Resolution with Overlapping Rules}
\label{sec:resolution}

An essential property of resolution is \textit{coherence}, which ensures that
the result of resolution is predictable and consistent. Incoherent programs,
where resolution cannot be resolved unambiguously, should be rejected.

%- - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
\subsection{Overlap}
Overlapping rules are a well-known source of incoherence. Consider
\begin{equation*}
\left\{ \forall \alpha. \alpha \rightarrow \tyint,  
        \forall \alpha. \tyint \rightarrow \alpha \right\} \vturns \tyint \rightarrow \tyint
\end{equation*}
Both the first and the second rule can be used to discharge this judgement.
In general, we have incoherence when there are multiple possible resolution derivations.

In order to avoid incoherence, existing approaches in the literature take a the
Draconian measure of forbidding overlap altogether. However, overlap
is a highly useful features, as illustrated by the many practical
applications in GHC/Haskell.\footnote{despite the fact that Haskell
implementations do not truly rule out incoherence}
Hence, we adopt a less conservative approach.

%- - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
\subsection{Overlap Resolution}
To avoid the potential incoherence, we provide a two-level priority scheme to
specify which one of several overlapping rules is selected during resolution. 

The first priority is the natural priotirization in the implicit environment.
This environment behaves as a stack of sets. A rule in a set closer to the top
of the stack has priority over one further down in the stack. For instance,
\begin{equation*}
\left\{ \forall \alpha. \alpha \rightarrow \tyint \right\},  
\left\{ \forall \alpha. \tyint \rightarrow \alpha \right\} \vturns \tyint \rightarrow \tyint
\end{equation*}
is uniquely resolved using the second rule, which is at the top of the stack.

The second level, in case of
overlapping rules within the same set in the implicit environment, is to
select the most specific matching rule. For instance,
\begin{equation*}
\left\{ \forall \alpha. \alpha \rightarrow \alpha,  
        \forall \alpha. \alpha \rightarrow \tyint \right\} \vturns \tyint \rightarrow \tyint
\end{equation*}
is uniquely resolved using the second rule, which is more specific than the first.

While this approach allows us to make effective use of overlapping rules in many
cases, we must still avoid situations where no most specific rule can be determined,
such as the first example.
This overlap resolution also raises concerns with respect to type safety. Consider:
\begin{equation*}
\left\{ \forall \alpha. \alpha \rightarrow \alpha,  
        \{\textit{Char}\} \To  \tyint \rightarrow \tyint \right\} \vturns \beta \rightarrow \beta
\end{equation*}
Regardless of whether $\beta$ is \tyint or not, there is a rule to select
in the implicit environment. However, when $\beta$ is \tyint, resolution
gets stuck, because there is no rule to produce a value of type \texttt{Char}.
In contrast, resolution does not get stuck for other instantiations.
As we wish to claim that well-typed programs do not get stuck, we need to make
sure that situations like this do not happen. 

%- - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\subsection{Condition Specifications} 

In order to avoid unsafe and incoherent overlap in a ruleset, we impose three
conditions.

%~~~
\paragraph{Most Specific Rule}
Firstly, there must always be a most specific rule.
\begin{definition}[Existence of Most Specific Rule Condition]
We say that a ruleset $\pi$ always has a most specific rule iff
\[
\begin{array}{l}
  \forall \theta.\forall \tau.\rho_1,\rho_2\in\pi.
  \theta|\rho_1| \succeq \theta\tau \wedge \theta|\rho_2| \succeq \theta\tau \\
  \implies \exists \rho \in \pi. \theta|\rho| = \theta(|\rho_1| \sqcap |\rho_2|)
\end{array}
\]
We use $\mathit{exists}(\pi)$ to denote such ruleset.
\end{definition}

Note that the order between types can be affected by type type substitution.
A pair of types on which no order relationship exists may have an order after 
applying substiution. So we have to consider every possible substitutions.
See following example.
\[
\{
  \forall \alpha. \alpha \rightarrow {\tt int} \rightarrow a,
  \forall \alpha. {\tt int} \rightarrow \alpha  \rightarrow {\tt int} 
\} 
\vturns {\tt int} \rightarrow {\tt int} \rightarrow {\tt int}
\]

The resolution will be ambiguous if type variable $a$ is substituted with ${\tt int}$.

%~~~
\paragraph{Uniqueness}
Secondly, the most specific instance must be unique. This avoids situations
where multiple rules \textit{statically} have the same result type.
\begin{equation*}
\left\{ \texttt{int}, \texttt{char} \Rightarrow \texttt{int}, \texttt{char} \right\} 
\vturns \texttt{int}
\end{equation*}
However, we should also consider the effect of a type substitution, and make
sure that uniqueness remains true \textit{dynamically}. Consider this case:
\begin{equation*}
\left\{ \alpha, \tyint \right\} \vturns \tyint
\end{equation*}
It statically appears that the second is the only appropriate one to resolve
\tyint. However, at runtime, the type variable $\alpha$ may well be
instantiated to \tyint, which would mean that there are actually two
implicit \tyint values.

The following condition makes sure of both static and dynamic uniqueness.
\begin{definition}[Uniqueness of Instances]
We say that the ruleset $\pi$ is consistent with unique instances iff 
\[
\forall \rho_1,\rho_2 \in \pi, \theta. 
  \rho_1 \neq \rho_2
  \implies \theta |\rho_1| \neq \theta |\rho_2|
\]
We use $\mathit{unique}(\pi)$ to denote such ruleset.
\end{definition}

%~~~
\paragraph{Type Safety}
We must ensure that every resolution that succeeds for a general type also
succeeds for a more specific type.
\begin{definition}[Type Safety Condition]
An implicit environment $\env$ is type safe iff
\begin{equation*}
\forall \rulet, \theta  . \env \vturns \rulet \wedge \mathit{dom}(\theta) = \mathit{fv}(\rulet) \cup \mathit{fv}(\env)
~~\Longrightarrow~~ 
\theta\env \vturns \theta\rulet
\end{equation*}
\end{definition}

We may need restricted algorithmic check. Naively restricting specific instances to
have less constraint then general instances will not work. Assume we have the most
general pretty printer that prints $``\dots''$ for any input and polymorphic pretty
printer for lists which takes a pretty printer for an elemetns type implicitly.
A program having such pretty printers is natural but it will be rejected by naive
restriction 

\tom{Algorithm}


%~~~
\paragraph{Coherent Environment} We now combine the above conditions
on rulesets and extend them to environments.
\begin{theorem}[Coherent Environment]
An environment $\env$ has a unique most specific instance for any query if
every stack element of the environment has unique most specific instances.
\tom{formal statement}
\end{theorem}
\wt{PROOF}

%-------------------------------------------------------------------------------
\subsection{Static Condition Checking}

We have formulated coherence conditions on the implicit environment, but not
yet stated where in the type system these conditions are imposed.

One approach is to impose the conditions throughout, on every 
environment and ruleset in all type system rules. This approach not only burdens the
formulation of the type system, it also unnecessarily rejects many useful
programs, like the following rule\footnote{similar to 
an \texttt{instance (C a, C b) => C (a,b)} of a type class \texttt{C} in Haskell}
\begin{equation*}
f \stackrel{\mathit{def}}{\equiv}\ruleabs{(\forall a,b.\{a,b\} \Rightarrow a \times b)}{(?a,?b)}
\end{equation*}
where $\{a,b\}$ violates the uniqueness condition (as $\theta a = \theta b$ for $\theta = [a \mapsto \type, b \mapsto \type]$). It would be a shame if we could
not use this rule in safe situations, like
\begin{equation*}
\ruleapp{f[\tyint,\texttt{Bool}]}{\{1:\tyint,\texttt{true}:\texttt{Bool}\}}
\end{equation*}
In the same vain, we would like to accept
\begin{equation*}
\ruleapp{f[\tyint,\tyint]}{\{1:\tyint\}}
\end{equation*}
where the substitution collapses the set of required implicit rules to a
singleton.
In order to avoid rejecting these programs, we must not check for uniqueness
at rule abstraction sites (\textbf{rule}), but defer them to a \textit{later} point.
In particular, we do want to reject programs like
\begin{equation*}
g \stackrel{\mathit{def}}{\equiv}
\ruleabs{(\forall a.\{a\} \Rightarrow a \times \tyint)}
      {\ruleapp
        {f[a,\tyint]}
        {\{?a:a,3:\tyint\}}}
\end{equation*}
which dynamically does not have a unique most general rule in a context like 
$\ruleapp{ g[\tyint]}{\{ 4 : \tyint\}}$. Deferring the check beyond
$g$'s definition leaves us with too little information. Hence, we must perform
the existence check at rule application (\textbf{with}).

Finally, we need another existence check at resolution ($?\rulet$). Consider
the program
\[\begin{array}{l}
\tstate \vturns 
\ruleapp{(?(\forall a.\{a\}\Rightarrow a \times \texttt{int}))[\texttt{int}]}
  {\{4:\texttt{int}\}}
\end{array}\]
where $\tstate = \{f:\forall a,b.\{a,b\}\Rightarrow (a, b) ,3:\texttt{int}\}$.
In this program, the two \texttt{int} values are supplied by different means to $f$,
$4$ through the \texttt{with} construct, but $3$ through recursive resolution. Hence,
the latter also requires a check.

\paragraph{Summary}
Our type system checks:  
\textit{existence} of most specific instances at rule definitions (\texttt{rule}), and
\textit{uniqueness} of instances at resolution ($?\rulet$) and rule application (\texttt{with}).
% If the ruleset in rule signatures statically ensures the existence of most specific instances, 
% then the runtime environment will always have most specific instances.
% Furthermore, if a static check prevents every attempt to make an environment with duplicate
% entries at rule application and sites, then we will always have unambiguous environments at runtime.
% There are only two such positions : rule applications and resolutions.

\begin{definition}[Coherent Program]
Program $e$ with type $\tau$ is coherent iff the following conditions hold throughout
the derivation tree of $\epsilon \turns e:\tau$.
\begin{itemize}
\item 
  For all subexpression $\ruleabs{\forall \overline{\alpha}.\pi\Rightarrow \tau}{e}$ :
    $\texttt{exists}(\pi)$
\item
  For all subexpression $\ruleapp{e}{\overline{e}:\overline{\rho}}$ :
    \mbox{$\texttt{unique}$}$(\overline{\rho})$
\item
  For all sub-derivations 
  $\Gamma \turns \forall \overline{\alpha}. \pi_1 \Rightarrow \tau$ :
    Assume $\Gamma(\forall \overline{\alpha}.\tau) 
    = \forall \overline{\beta}.\pi_2 \Rightarrow \tau_2$
    and $\theta$ is a substitution such that $\theta \tau_2 = \tau_1$.
    The the followings should hold : $\texttt{unique}(\theta\pi_2 - \pi_1)$
    and $\forall \rho_1 \in \pi_1.\rho_2 \in \pi_2. \theta\rho_2 \nsucceq \rho_1$.
\end{itemize}
\end{definition}


% Statically checking an argument at rule application sites is enough 
% to reject following ambiguous program. 
% \[\begin{array}{l}
% \texttt{let } f=\ruleabs{(\forall a,b.\{a,b\} \Rightarrow a \times b)}{(?a,?b)} \\
% \texttt{in let } g=
%   {\ruleabs{(\forall a.\{a\} \Rightarrow a \times \texttt{int})}
%     {\ruleapp
%       {f[a,\texttt{int}]}
%       {\{?a,3\}}}} \\
% \texttt{in } \ruleapp{g[\texttt{int}]}{\{4\}}
% \end{array}\]

% Static check at a resolution site can also prevent following ambiguous program.
% Let $I = \{(?a,?b):\forall a,b.\{a,b\}\Rightarrow a \times b  ,3:\texttt{int}\}$
% \[\begin{array}{l}
% I \vturns 
% \ruleapp{(\forall a.\{a\}\Rightarrow a \times \texttt{int})[\texttt{int}]}
%   {\{4:\texttt{int}\}}
% \end{array}\]

% Our checking algorithm can accept following case since we delay unambiguouty check to
% the use point.
% \[
% \ruleapp
%   {(\ruleabs{\forall a,b.\{a,b\} \Rightarrow (a,b)}{(?a,?b)})
%     [\texttt{int},\texttt{int}]}
%   {\{3:\texttt{int}\}}
% \]

\wt{THEOREM : Type Safe Program Never Generates Ambiguous Environment}
\tom{The theorem should just be type saftey.}
\wt{Mentioning other possible options}

%\begin{definition}[Most Specific Rule Condition]
%We say that an environment $\env$ always has a most specific rule iff
%\begin{multline*}
%\forall \tau.
%\forall \rho_1, 
%        \rho_2 \in \env^*(\tau).
%        \exists (\rulesch{\alpha_3}{\ruleset_3}{\tau_3}) \in \env^{*}(\tau).\\
%        \{\rho_1,\rho_2\} \subseteq \env^*(\tau_3)
%\end{multline*}
%where
%\begin{equation*}
%\left\{\begin{array}{rcl}
%(\env,\bar{\rho})^*(\tau) & = & \{(\rulesch{\alpha'}{\ruleset'}{\tau'}) \in \bar{\rho} \mid \tau \preceq_{\bar{\alpha}'} \tau' \} \lhd \env^*(\tau)\\
%\epsilon^*(\tau)          & = & \emptyset 
%\end{array}\right.
%\end{equation*}
%with
%\begin{equation*}
%\left\{\begin{array}{rcl}
%\emptyset \lhd \bar{\rho}_2      & = & \bar{\rho}_2\\
%\bar{\rho}_1 \lhd \bar{\rho}_2   & = & \bar{\rho}_1 \hspace{1cm}, \rho_1 \neq \emptyset
%\end{array}\right.
%\end{equation*}
%and
%begin{equation*}
%
%\tau_1 \preceq_{\bar{\alpha}} \tau_2 \stackrel{\mathit{def}}{\Longleftrightarrow}  
%\exists \bar{\tau}. [\bar{\alpha} \mapsto \bar{\tau}]\tau_2 = \tau_1
%\end{equation*}
%\end{definition}
%
%\tom{define lookup}
%
%
%The above condition only makes sure that every most step in the recursive
%resolution process either fails or succeeds deterministically.
%
%% and
%% \begin{multline*}
%% \forall (\rulesch{\alpha_1}{\kappa_1}{\ruleset_1}{\tau_1}), 
%%         (\rulesch{\alpha_2}{\kappa_2}{\ruleset_2}{\tau_2}) \in \ruleset.\\
%%         \tau_2 \preceq \tau_1 \wedge
%%         \tau_1 \preceq \tau_2 \Longrightarrow \\
%%         \rulesch{\alpha_1}{\kappa_1}{\ruleset_1}{\tau_1} = 
%%         \rulesch{\alpha_2}{\kappa_2}{\ruleset_2}{\tau_2}
%% \end{multline*}
%
%

%- - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
\subsection{Operational versus Elaboration Semantics}
Our informal notion of coherent overlap always allows us to select
the appropriate implicit rule \textit{at runtime}, which is perfect
for the operational semantics.
Not so for the elaboration semantics, which (by definition) has to select the
appropriate rule statically. For instance,
\begin{equation*}
\left\{ \forall \alpha. \alpha \rightarrow \alpha,  
        \tyint \rightarrow \tyint \right\} \vturns \beta \rightarrow \beta
\end{equation*}
Statically, we do not know whether $\beta$ equals \tyint or not.  For the
operational semantics this is fine: statically we only check that there is a
unique resolution in both cases. At runtime we will know which of these to
chose, as the type variable $\beta$ will be instantiated.
However, the elaboration semantics must chose at compile time, and thus cannot
resolve this situation.  

As a consequence, the elaboration semantics is forced to accept fewer programs
than the operational semantics.  In particular, if we insist that the implicit
environment is able to resolve every possible query coherently, then the
elaboration semantics cannot tolerate any overlap at all. A more liberal
approach only considers whether the queries $\env \vturns \rulet$ that actually
appear in the program (originating from the $?\rulet$ construct) are resolved
coherently. GHC takes a similar approach for overlapping type class instances,
yet coherence is not guaranteed across multiple modules. Note that only
checking coherence for program queries also makes sense for the operational
semantics.



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../Main"
%%% End: 


==> src/Semantics.tex <==

%% ODER: format ==         = "\mathrel{==}"
%% ODER: format /=         = "\neq "
%
%
\makeatletter
\@ifundefined{lhs2tex.lhs2tex.sty.read}%
  {\@namedef{lhs2tex.lhs2tex.sty.read}{}%
   \newcommand\SkipToFmtEnd{}%
   \newcommand\EndFmtInput{}%
   \long\def\SkipToFmtEnd#1\EndFmtInput{}%
  }\SkipToFmtEnd

\newcommand\ReadOnlyOnce[1]{\@ifundefined{#1}{\@namedef{#1}{}}\SkipToFmtEnd}
\usepackage{amstext}
\usepackage{amssymb}
\usepackage{stmaryrd}
\DeclareFontFamily{OT1}{cmtex}{}
\DeclareFontShape{OT1}{cmtex}{m}{n}
  {<5><6><7><8>cmtex8
   <9>cmtex9
   <10><10.95><12><14.4><17.28><20.74><24.88>cmtex10}{}
\DeclareFontShape{OT1}{cmtex}{m}{it}
  {<-> ssub * cmtt/m/it}{}
\newcommand{\texfamily}{\fontfamily{cmtex}\selectfont}
\DeclareFontShape{OT1}{cmtt}{bx}{n}
  {<5><6><7><8>cmtt8
   <9>cmbtt9
   <10><10.95><12><14.4><17.28><20.74><24.88>cmbtt10}{}
\DeclareFontShape{OT1}{cmtex}{bx}{n}
  {<-> ssub * cmtt/bx/n}{}
\newcommand{\tex}[1]{\text{\texfamily#1}}	% NEU

\newcommand{\Sp}{\hskip.33334em\relax}


\newcommand{\Conid}[1]{\mathit{#1}}
\newcommand{\Varid}[1]{\mathit{#1}}
\newcommand{\anonymous}{\kern0.06em \vbox{\hrule\@width.5em}}
\newcommand{\plus}{\mathbin{+\!\!\!+}}
\newcommand{\bind}{\mathbin{>\!\!\!>\mkern-6.7mu=}}
\newcommand{\rbind}{\mathbin{=\mkern-6.7mu<\!\!\!<}}% suggested by Neil Mitchell
\newcommand{\sequ}{\mathbin{>\!\!\!>}}
\renewcommand{\leq}{\leqslant}
\renewcommand{\geq}{\geqslant}
\usepackage{polytable}

%mathindent has to be defined
\@ifundefined{mathindent}%
  {\newdimen\mathindent\mathindent\leftmargini}%
  {}%

\def\resethooks{%
  \global\let\SaveRestoreHook\empty
  \global\let\ColumnHook\empty}
\newcommand*{\savecolumns}[1][default]%
  {\g@addto@macro\SaveRestoreHook{\savecolumns[#1]}}
\newcommand*{\restorecolumns}[1][default]%
  {\g@addto@macro\SaveRestoreHook{\restorecolumns[#1]}}
\newcommand*{\aligncolumn}[2]%
  {\g@addto@macro\ColumnHook{\column{#1}{#2}}}

\resethooks

\newcommand{\onelinecommentchars}{\quad-{}- }
\newcommand{\commentbeginchars}{\enskip\{-}
\newcommand{\commentendchars}{-\}\enskip}

\newcommand{\visiblecomments}{%
  \let\onelinecomment=\onelinecommentchars
  \let\commentbegin=\commentbeginchars
  \let\commentend=\commentendchars}

\newcommand{\invisiblecomments}{%
  \let\onelinecomment=\empty
  \let\commentbegin=\empty
  \let\commentend=\empty}

\visiblecomments

\newlength{\blanklineskip}
\setlength{\blanklineskip}{0.66084ex}

\newcommand{\hsindent}[1]{\quad}% default is fixed indentation
\let\hspre\empty
\let\hspost\empty
\newcommand{\NB}{\textbf{NB}}
\newcommand{\Todo}[1]{$\langle$\textbf{To do:}~#1$\rangle$}

\EndFmtInput
\makeatother
%
%
%
% First, let's redefine the forall, and the dot.
%
%
% This is made in such a way that after a forall, the next
% dot will be printed as a period, otherwise the formatting
% of `comp_` is used. By redefining `comp_`, as suitable
% composition operator can be chosen. Similarly, period_
% is used for the period.
%
\ReadOnlyOnce{forall.fmt}%
\makeatletter

% The HaskellResetHook is a list to which things can
% be added that reset the Haskell state to the beginning.
% This is to recover from states where the hacked intelligence
% is not sufficient.

\let\HaskellResetHook\empty
\newcommand*{\AtHaskellReset}[1]{%
  \g@addto@macro\HaskellResetHook{#1}}
\newcommand*{\HaskellReset}{\HaskellResetHook}

\global\let\hsforallread\empty

\newcommand\hsforall{\global\let\hsdot=\hsperiodonce}
\newcommand*\hsperiodonce[2]{#2\global\let\hsdot=\hscompose}
\newcommand*\hscompose[2]{#1}

\AtHaskellReset{\global\let\hsdot=\hscompose}

% In the beginning, we should reset Haskell once.
\HaskellReset

\makeatother
\EndFmtInput
%
%
%
%
%
% This package provides two environments suitable to take the place
% of hscode, called "plainhscode" and "arrayhscode". 
%
% The plain environment surrounds each code block by vertical space,
% and it uses \abovedisplayskip and \belowdisplayskip to get spacing
% similar to formulas. Note that if these dimensions are changed,
% the spacing around displayed math formulas changes as well.
% All code is indented using \leftskip.
%
% Changed 19.08.2004 to reflect changes in colorcode. Should work with
% CodeGroup.sty.
%
\ReadOnlyOnce{polycode.fmt}%
\makeatletter

\newcommand{\hsnewpar}[1]%
  {{\parskip=0pt\parindent=0pt\par\vskip #1\noindent}}

% can be used, for instance, to redefine the code size, by setting the
% command to \small or something alike
\newcommand{\hscodestyle}{}

% The command \sethscode can be used to switch the code formatting
% behaviour by mapping the hscode environment in the subst directive
% to a new LaTeX environment.

\newcommand{\sethscode}[1]%
  {\expandafter\let\expandafter\hscode\csname #1\endcsname
   \expandafter\let\expandafter\endhscode\csname end#1\endcsname}

% "compatibility" mode restores the non-polycode.fmt layout.

\newenvironment{compathscode}%
  {\par\noindent
   \advance\leftskip\mathindent
   \hscodestyle
   \let\\=\@normalcr
   \let\hspre\(\let\hspost\)%
   \pboxed}%
  {\endpboxed\)%
   \par\noindent
   \ignorespacesafterend}

\newcommand{\compaths}{\sethscode{compathscode}}

% "plain" mode is the proposed default.
% It should now work with \centering.
% This required some changes. The old version
% is still available for reference as oldplainhscode.

\newenvironment{plainhscode}%
  {\hsnewpar\abovedisplayskip
   \advance\leftskip\mathindent
   \hscodestyle
   \let\hspre\(\let\hspost\)%
   \pboxed}%
  {\endpboxed%
   \hsnewpar\belowdisplayskip
   \ignorespacesafterend}

\newenvironment{oldplainhscode}%
  {\hsnewpar\abovedisplayskip
   \advance\leftskip\mathindent
   \hscodestyle
   \let\\=\@normalcr
   \(\pboxed}%
  {\endpboxed\)%
   \hsnewpar\belowdisplayskip
   \ignorespacesafterend}

% Here, we make plainhscode the default environment.

\newcommand{\plainhs}{\sethscode{plainhscode}}
\newcommand{\oldplainhs}{\sethscode{oldplainhscode}}
\plainhs

% The arrayhscode is like plain, but makes use of polytable's
% parray environment which disallows page breaks in code blocks.

\newenvironment{arrayhscode}%
  {\hsnewpar\abovedisplayskip
   \advance\leftskip\mathindent
   \hscodestyle
   \let\\=\@normalcr
   \(\parray}%
  {\endparray\)%
   \hsnewpar\belowdisplayskip
   \ignorespacesafterend}

\newcommand{\arrayhs}{\sethscode{arrayhscode}}

% The mathhscode environment also makes use of polytable's parray 
% environment. It is supposed to be used only inside math mode 
% (I used it to typeset the type rules in my thesis).

\newenvironment{mathhscode}%
  {\parray}{\endparray}

\newcommand{\mathhs}{\sethscode{mathhscode}}

% texths is similar to mathhs, but works in text mode.

\newenvironment{texthscode}%
  {\(\parray}{\endparray\)}

\newcommand{\texths}{\sethscode{texthscode}}

% The framed environment places code in a framed box.

\def\codeframewidth{\arrayrulewidth}
\RequirePackage{calc}

\newenvironment{framedhscode}%
  {\parskip=\abovedisplayskip\par\noindent
   \hscodestyle
   \arrayrulewidth=\codeframewidth
   \tabular{@{}|p{\linewidth-2\arraycolsep-2\arrayrulewidth-2pt}|@{}}%
   \hline\framedhslinecorrect\\{-1.5ex}%
   \let\endoflinesave=\\
   \let\\=\@normalcr
   \(\pboxed}%
  {\endpboxed\)%
   \framedhslinecorrect\endoflinesave{.5ex}\hline
   \endtabular
   \parskip=\belowdisplayskip\par\noindent
   \ignorespacesafterend}

\newcommand{\framedhslinecorrect}[2]%
  {#1[#2]}

\newcommand{\framedhs}{\sethscode{framedhscode}}

% The inlinehscode environment is an experimental environment
% that can be used to typeset displayed code inline.

\newenvironment{inlinehscode}%
  {\(\def\column##1##2{}%
   \let\>\undefined\let\<\undefined\let\\\undefined
   \newcommand\>[1][]{}\newcommand\<[1][]{}\newcommand\\[1][]{}%
   \def\fromto##1##2##3{##3}%
   \def\nextline{}}{\) }%

\newcommand{\inlinehs}{\sethscode{inlinehscode}}

% The joincode environment is a separate environment that
% can be used to surround and thereby connect multiple code
% blocks.

\newenvironment{joincode}%
  {\let\orighscode=\hscode
   \let\origendhscode=\endhscode
   \def\endhscode{\def\hscode{\endgroup\def\@currenvir{hscode}\\}\begingroup}
   %\let\SaveRestoreHook=\empty
   %\let\ColumnHook=\empty
   %\let\resethooks=\empty
   \orighscode\def\hscode{\endgroup\def\@currenvir{hscode}}}%
  {\origendhscode
   \global\let\hscode=\orighscode
   \global\let\endhscode=\origendhscode}%

\makeatother
\EndFmtInput
%


\section{The $\ourlang$ Calculus}
\label{sec:ourlang}

This section presents the syntax and operational semantics 
of $\ourlang$. Our calculus $\ourlang$ combines standard scoping mechanisms 
(abstractions and applications) and types \`a la System F, with a
logic-programming-style query language. 
At the heart of the language is a threefold interpretation of types:
\begin{center}
  \ensuremath{\Varid{types}\cong\Varid{propositions}\cong\Varid{rules}}
\end{center}
\noindent Firstly, types have their traditional meaning of classifying
values.  Secondly, via the Curry-Howard isomorphism, types can
also be interpreted as propositions -- in the context of IP, the type
proposition denotes the availability in the implicit environment of a
value of the corresponding type. Thirdly, a type is interpreted as a
logic-programming style rule, i.e., a Prolog rule or Horn
clause~\cite{kowalski}.
%%\footnote{The connection between type class
%%  instances and Prolog rules is folklore.}
Resolution~\cite{resolution} connects rules and propositions: it is
the means to show (the evidence) that a proposition is entailed by a set of rules.
%%Again, a value serves as evidence for the rule interpretation,
%%constructing a proof of one proposition in terms of proofs of others.

%-------------------------------------------------------------------------------
\subsection{Syntax}    
\label{subsec:syntax}
%%$\ourlang$ is a minimal calculus that models a query language,
%%resembling a simple logic programming language. 

The syntax of the calculus is shown next:
{\small \bda{llrl}
    \text{Types} & \type \hide{\in \meta{Type}} & ::=  & \alpha \mid \rulet \\
    \text{Rule Types} & \rulet \hide{\in \meta{RType}} & ::= & 
    \rulesch{\alpha}{\rulesetvar}{\type} \\
    \text{Context} & \rulesetvar \hide{\in 2^\meta{RType}} & ::= & 
    \nil \mid \bar{\rulet} \\
    \text{Expressions} & \ensuremath{\Varid{e}} & ::=  &
    \ensuremath{?\!\rulet} \mid 
    \ensuremath{\ruleabs{\rulet}{\Varid{e}}} \mid
    e[\bar{\type}] \mid
    \ensuremath{\Varid{e}\;{\bf with}\;\rulesetexp} \\
  \eda }
Types $\type$ are either type variables $\alpha$ or rule types
$\rulet$.  A rule type $\rho = \rulesch{\alpha}{\rulesetvar}{\type}$
is a type scheme with universally quantified variables $\bar{\alpha}$
and an (implicit) context $\rulesetvar$. We use an overline
to denote a set of entities, like $\bar{\alpha}$. The context is simply 
a set of rule types, which summarizes the assumed implicit environment. We
usually omit empty universal quantifiers and contexts from a rule
type. 

There are four forms of expression. A query \ensuremath{?\!\rulet} queries
the implicit environment for a value of type $\rulet$.  A rule
abstraction \\ \ensuremath{\ruleabs{\rulesch{\alpha}{\rulesetvar}{\type}}{\Varid{e}}} builds a rule whose type is \ensuremath{\rulesch{\alpha}{\rulesetvar}{\type}}
and whose body is $e$. Rule abstraction has double roles as
a binding structure: 1) the universal quantification of type variables
binds types, and 2) the context binds a rule set. These binders are
respectively eliminated by type application $e[\bar{\type}]$ and rule
application \ensuremath{\Varid{e}\;{\bf with}\;\rulesetexp}. 
% \hide{\bruno{old explanation here.} The main reason why we merged
% two binding structures into one is that we need the information of
% type variables and context at the same time when we match a rule in
% resolution. If we split a rule into multiple constructs, the
% resolution becomes very complex.}

While System F traditionally separates type and value binders in separate
constructs $\Lambda$ and $\lambda$, they belong naturally together in our
interpretation of rules as logic programming rules.\footnote{In Prolog these
are not separated either.} After all, in the matching process of resolution, a
rule is applied as a unit.  Hence, separating rules into more primitive binders
(\`a la System F's type and value binders) would only complicate the definition
of resolution unnecessarily.

% Following the
% interpretation of types as rules, a rule type $\forall \bar{\alpha}.\pi \To
% \type$ combines 3 components: a universal quantifier of type variables
% $\bar{\alpha}$, a left-hand side $\pi$ of assumptions and a right-hand side
% $\type$ which is the consequent of the rule.
% %
% While these three components belong naturally together in $\ourlang$, they
% would be separated in System F, which does not assume a rule interpretation of
% types. Indeed, in System F, a rule like
% 
% %{
% 
% %format blambda = "\Lambda\!"
% %format # = "."
% 
% > rule (forall a b . {a,b} => Pair a b) ((query (Pair a b)))
% 
% would correspond to a term like:
% 
% > blambda a # blambda b # \(x : a) # \(y : b) # (x,y) 



For brevity $\ourlang$ only concerns IP constructs. In examples we
often use additional syntax such as $\lambda$-binders, integer
and boolean literals and their corresponding types. Extending this
calculus with support for \emph{higher-kinded polymorphism} in the
style of System $F_{\omega}$ is straightforward.  The implementation
of the source language (and $\ourlang$) presented in
Section~\ref{sec:example} implements various of these extensions.

%-------------------------------------------------------------------------------


% or lead to ad-hoc designs of resolution with potential loss of
% expressiveness. 


%-------------------------------------------------------------------------------
\subsection{Operational Semantics}
\label{subsec:opsem}

\figtwocol{fig:opsem}{Operational Semantics}{
\small
\bda{lc} 

\multicolumn{2}{l}{\myruleform{\tstate \turns e \eval v}} \\

\OpQuery &
\myirule
{ \tstate \vturns \rulet \eval v}
{ \tstate \turns ?\rulet \eval v }
\\ \\

\OpRule &
\myirule
{}
{ \tstate \turns \ruleabs{\rulet}{e} \eval 
  \rclos{\rulet, e, \tstate, \shade{\nil}}}
 \\ \\

\OpInst &
\myirule
{ \tstate \turns e \eval 
  \rclos{\rulet', e', \tstate', \shade{\rulepgmvar'}} \\
  \rulet' \leteq \rulesch{\alpha}{\rulesetvar}{\type} 
}
{ \tstate \turns e[\bar{\type}] \eval 
  \subst{\overline{\alpha}}{\overline{\type}}
  \rclos{\rulesetvar \To \type, e', \tstate', \shade{\rulepgmvar'}}
} \\ \\

\OpRApp &
\myirule
{ \tstate \turns e \eval 
  \rclos{\rulet', e', \tstate', \shade{\rulepgmvar'}} \\
  \tstate \turns e_i \eval v_i \quad
  (\forall \relation{e_i}{\rulet_i} \in \rulesetexp) \\
  \tstate'; \rulepgm \shade{\cup~\rulepgmvar'} \turns e' \eval v
}
{ \tstate \turns \ruleapp{e}{\rulesetexp} \eval v
} \\ \\

\multicolumn{2}{l}{\myruleform{\tstate \vturns \rulet \eval v}} \\

\DynRes &
\myirule
{ \lookup{\tstate}{\type} =
  \rclos{\rulesch{\beta}{\pi'}{\type'}, e', 
    \tstate', \shade{\rulepgmvar'}} \\ 
  \rulet \leteq \rulesch{\alpha}{\shade{\pi}}{\type} \quad
  \theta \leteq \unify{\type'}{\type}{\bar{\beta}} \\
  \tstate \vturns \rulet_i \eval v_i \quad 
  (\forall \rulet_i \in \theta \pi' \shade{-~\pi})
}
{ \tstate \vturns \rulet \eval 
  \rclos{\rulet, \theta e', \theta \tstate', 
    \rulepgm \shade{\cup ~ \theta \rulepgmvar'}}
} \\ \\
\eda

\bda{llc}

\multicolumn{1}{l}{\myruleform{\lookup{\tstate}{\type} = v}}
& & \myirule
{
  \lookup{\rulepgmvar}{\type} = v
}
{
  \lookup{(\tstate;\rulepgmvar)}{\type} = v
} \quad

\myirule
{
  \lookup{\rulepgmvar}{\type} = \bot \quad
  \lookup{\tstate}{\type} = v
}
{
  \lookup{(\tstate;\rulepgmvar)}{\type} = v
} \\ \\ 

\multicolumn{1}{l}{\myruleform{\lookup{\rulepgmvar}{\type} = v}} 
& & \myirule
{
  (\rulet:v) \in \rulepgmvar \quad
  \rulet \succ \type \\
  \not \exists (\rulet':v') \in \rulepgmvar. 
  \rulet' \succ \type \wedge (\rulet:v) \neq (\rulet':v'')
}
{
  \lookup{\rulepgmvar}{\type} = v
} \\ \\

& & \myirule
{
  \forall (\rulet:v) \in \rulepgmvar. \rulet \nsucc \type 
}
{
  \lookup{\rulepgmvar}{\type} = \bot
}
\eda
}

The operational semantics, given in Figure \ref{fig:opsem}, is a
call-by-value big-step operational semantics. The judgment $\tstate
\turns e \eval v$ means, as usual, that expression $e$ evaluates to
value $v$ under environment $\tstate$.
{\small
\bda{llrl} 
\text{Values (Closures)} & v \hide{\in \meta{Val}} & ::= &
\rclos{\rulet, e, \tstate, \rulepgmvar} \\
\text{Environments} & \tstate \hide{\in \meta{Env}} & ::= &
\cdot \mid \tstate; \rulepgmvar \\
\text{Rule sets} & \rulepgmvar \hide{\in \meta{Pgm}} & ::= &
\nil \mid \rulepgm \\
\eda 
}
An environment $\tstate$ is a stack of {\it rule sets}. Each rule set
is a set of mappings from rule types to corresponding values. The
stack nature of an environment captures the lexical scope of different
rules.

% In the following example, the
% environment at {\tt (*1*)} is
% $\myset{\relation{\tyint}{1}};\myset{\relation{\tyint}{2}}$:
% \Ex{
%   f = \ruleabs{(\myset{\tyint} \To \tyint)}{(?\tyint)} \\
%   \ruleapp
%   {\ruleapp
%     {f {\tt (* 1 *)} }
%     {\myset{\relation{2}{\tyint}}}}
%   {\myset{\relation{1}{\tyint}}}
% }
% \tom{Fix the above example.}
% The impact of scoping becomes clear when we discuss resolution in section
% \ref{sec:resolution}.

The only values in $\ourlang$ are closures of rule abstractions.
Such a closure $\rclos{\rulet, e, \tstate, \rulepgmvar}$ consists of 
its type $\rulet$, rule body $e$, captured environment $\tstate$ and partially
resolved context $\rulepgmvar$. %%, which is explained shortly.

The operational semantics is syntax-directed. The gray parts of the
operational semantics relate to the partially resolved contexts and can be
ignored for now; we explain
them later.  Rule $\OpRule$ builds a closure from a rule abstraction
in the obvious way.  Rule $\OpInst$ substitutes formal type parameters
by the actually supplied types.  
%Substitution on types, rule types,
%expressions, values, rule programs and environments is formally
%defined in Figure~\ref{fig:subst}. 
Here $\substone$ is a substitution
from type variable $\alpha$ to $\type$ and
$\subst{\bar{\alpha}}{\bar{\type}}$ is a simultaneous substitution of
$[\alpha_1\!\mapsto\!\type_1, \cdots,
\alpha_n\!\mapsto\!\type_n]$.
Finally, rule $\OpRApp$ supplies the
required evidence for the assumptions of a rule closure and evaluates
the rule body to a value.

%- - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
\paragraph{Resolution}
Rule $\OpQuery$ defines the semantics of queries in terms of auxiliary
judgment $\tstate \vturns \rulet \eval v$, which expresses that rule
type $\rulet$ resolves to $v$ with respect to~$\tstate$.

The underlying principle of (recursive) resolution in $\ourlang$ (and
IP in general) originates from resolution in logic. We assign to each
rule type $\rulet$ a logical interpretation denoted $\rulet^\dagger$:
\begin{eqnarray*}
(\forall \bar{\alpha}.\pi \To \type)^\dagger & = & \forall \bar{\alpha} . \bigwedge_{\rho \in \pi} \rho^\dagger \To \type^\dagger
\end{eqnarray*}
and base types are interpreted as ``there is an implicit value of this type''.
Closures provide the necessary runtime evidence.
% For instance, \textit{rule type} |{Bool} => Int| has logical interpretation $|Bool| \Rightarrow |Int|$.
% In this example, the formula is a Horn clause,\footnote{ ``\texttt{int
% :- bool.}'' in Prolog syntax} but in general implications nest to the left.
Resolution in $\ourlang$ then corresponds to checking entailment of the logical interpretation:
\begin{center}
If $\tstate \vturns \rho \eval v$, then $\tstate^\dagger \models \rho^\dagger$.
\end{center}
Rule $\DynRes$ defines resolution recursively.  First, it looks up a closure
with \textit{matching} rule type (see below for the definition of lookup).
Matching means that the right-hand side $\type'$ of the rule type can be instantiated to
the right-hand side $\type$ of the queried type using a one-way unifier $\theta$.  The
closure type's left-hand side $\theta\pi'$ %, minus the queried LHS $\ruleset$, 
is resolved recursively.  Finally, a ``patched'' form of the closure is returned:
the queried type is provided and the type substitution $\theta$ is applied. 
% and the newly resolved part of the context is added.

%%\bruno{Don't forget to fill in the dots!}
%%This definition of resolution is a \textit{conservative approximation} of
%%logical entailment on several accounts: ...

% Resolution is driven by the interpretation of 
% rule types as first-order logic formulas. This interpretation, denoted $(\cdot)^\dagger$,
% is defined as:
% \begin{eqnarray*}
% (\forall \bar{\alpha}.\pi \To \type)^\dagger & = & \forall \alpha . \bigwedge_{\rho \in \pi} \rho^\dagger \To \type^\dagger \\
% \tstate^\dagger & = & \{ \rho^\dagger \mid (\rho:v) \in \tstate \}
% \end{eqnarray*}
% Resolution conservatively approximates logical entailment:
% \begin{theorem}
% If $\tstate \vturns \rho \eval v$, then $\tstate^\dagger \models \rho^\dagger$.
% \end{theorem}
% The opposite does not hold for two reasons. Firstly, and most importantly, the
% value-level evidence of rule closures only supports left-to-right reasoning.
% Secondly, we restrict the power of recursive resolution to simplify reasoning
% about program behavior and properties. The logical interpretation of the recursive precondition
% of rule $\DynRes$ is:
% \[ \forall \rho^\dagger \in \theta\pi'^\dagger. \rho^\dagger \in \pi^\dagger \vee \tstate^\dagger \models \rho^\dagger \]
% which is stronger than the necessary condition:
% \[ \forall \rho^\dagger \in \theta\pi'^\dagger. \tstate^\dagger \wedge \pi^\dagger \models \rho^\dagger \]
% We return to the reason for this stronger condition \tom{later} when we investigate resolution in detail.

%- - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
\paragraph{Lookup}

% During dynamic query resolution, environment may have multiple rules match
% with given query. With in an environment, rules in a context nearest to the
% environment stack top is preferred. With in a context, we don't allow multiple
% matches. 

Figure \ref{fig:opsem} defines lookup of a type in environments
($\lookup{\tstate}{\type}$) and rule sets
($\lookup{\rulepgmvar}{\type}$).  Lookup in a rule set only yields a
result when it contains \textit{at most} one matching rule: it yields
the rule closure,\footnote{as in Prolog, quantified type variables should be renamed apart to
avoid variable capture}
if there is exactly one matching rule, and $\bot$ if
there is no matching rule.  Lookup in an environment, first looks in
the topmost rule set, and, in case of $\bot$, recursively looks in the
remainder of the environment.  

If a rule set contains multiple matching rules (overlapping rules),
the lookup is not defined.  Here,
$(\forall \bar{\alpha}.\pi \To
  \type') \succ \type \stackrel{\mathit{def}}{=} \exists \theta. \theta
  = \unify{\type'}{\type}{\bar{\alpha}}$,
where $\unify{\type'}{\type}{\bar{\alpha}}$ returns the most general
unifier of $\type'$ and $\type$ with its support set contained in
$\bar{\alpha}$.  Note that overlapping rules, which are allowed in
Haskell, can be modeled in $\ourlang$ using nested scoping, even
though they are not supported directly (see Section 5).



%- - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
\paragraph{Partially Resolved Contexts}
The partially resolved context $\rulepgmvar$ in the operational semantics
provides extra expressivity to deal with higher-order queries, i.e., $\tstate
\vturns \forall \bar{\alpha}.\pi \To \type \eval v$ where $\pi$ is non-empty.

Rule $\DynRes$ does not require an exact syntactic match $\unify{\pi'
  \To \type'}{\pi \To \type}{\bar{\beta}}$ between the queried
higher-order rule type and the one found in the environment. Instead,
there can be some remainder $\theta\pi' - \pi$ of the found rule,
which the query does not demand to be resolved right away. Hence, we
say that the found rule is \textit{partially resolved}. The evidence
for this partially resolved context is stored in the rule closure's
fourth component.

The partially resolved context is treated as follows: It starts out as
empty when a new closure is created in rule $\OpRule$. Then
(potentially multiple successive) applications of rule $\DynRes$ may
extend it: the part of the context that is not required by a
higher-order query is resolved and stored in the closure.  Finally,
rule $\OpRApp$ supplies the remainder of the context, adds it to the
front of the environment and evaluates the rule body. A non-empty
partially resolved context arises, for instance in the following
program:
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{3}{@{}>{\hspre}l<{\hspost}@{}}%
\column{5}{@{}>{\hspre}l<{\hspost}@{}}%
\column{7}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[3]{}\mathbf{let}\;\Varid{f}\mathrel{=}\ruleabs{\{\mskip1.5mu \Conid{Int},\Conid{Bool}\mskip1.5mu\}\Rightarrow \Conid{Int}}{\Varid{e}}\;\mathbf{in}{}\<[E]%
\\
\>[3]{}\hsindent{2}{}\<[5]%
\>[5]{}(\ruleabs{\rulet}{\mathbin{?}(\{\mskip1.5mu \Conid{Int}\mskip1.5mu\}\Rightarrow \Conid{Int})}\;{\bf with}\;{}\<[E]%
\\
\>[5]{}\hsindent{2}{}\<[7]%
\>[7]{}\{\mskip1.5mu \Varid{f}\mathbin{:}\{\mskip1.5mu \Conid{Int},\Conid{Bool}\mskip1.5mu\}\Rightarrow \Conid{Int},\Conid{True}\mathbin{:}\Conid{Bool}\mskip1.5mu\}){}\<[E]%
\ColumnHook
\end{hscode}\resethooks
where \ensuremath{\rulet\mathrel{=}\{\mskip1.5mu \{\mskip1.5mu \Conid{Int},\Conid{Bool}\mskip1.5mu\}\Rightarrow \Conid{Int},\Conid{Bool}\mskip1.5mu\}\Rightarrow (\{\mskip1.5mu \Conid{Int}\mskip1.5mu\}\Rightarrow \Conid{Int})}.
The resulting closure has the form 
$\rclos{\ensuremath{\{\mskip1.5mu \Conid{Int}\mskip1.5mu\}\Rightarrow \Conid{Int},\Varid{e},\mathbin{-},\{\mskip1.5mu \Conid{Bool}\mathbin{:}\Conid{True}\mskip1.5mu\}}}$.

% \begin{equation*}
% \myirule
% { \env(\type) = \ruleset' \To \type \\
%   \env, \ruleset \vturns \rulet_i' \quad
%   (\forall \rulet_i' \in \ruleset')
% }
% { \env \vturns \ruleset \To \type}
% \end{equation*}
% The recursive instance of this rule is more powerful.
% However, this more powerful rule extends the implicit environment. \ldots


% [TOM] This discussion belongs elsewhere. It is not about partial resolution
%       in particular, but resolution in general. Moreover, it concerns 
%       a surprising behavior that could be ruled out by the type system.
%       So I think it is more appropriate in the type system section.
%
% During partial resolution, subqueries may include uninstantiated type 
% variables. Their instantiation will be determined in future. 
% But until
% then, it will be safe to consider that they can be anything.
% Consider following example.
% \[\begin{array}{l}
%   \{ \forall a. a \rightarrow \tybool,\ 
%      \tyint \rightarrow \tybool,\ 
%      \forall a. \{a \rightarrow \tybool, a\times a\} \Rightarrow a\} \\
%   \turns (?\forall a.\{a \times a\}\Rightarrow a)[\tyint]
% \end{array}\]
% During the evaluation of the query part, the third rule will be taken at first.
% Then, to resolve difference between the query and the taken rule, 
% evaluation process have to resolve query $a \rightarrow \tybool$ type. 
% Since, we don't have enough type information, it will be safe to pick
% $\forall a.\rightarrow a \rightarrow \tybool$. 
% 
% Alternative is to detect cases where type information can be uncertain even
% at runtime and reject programs having such possibility using type system. 

% \wc{Figure on substitutions is moved to appendix}
% \tom{Where is it? I don't see it in the appendix}

\paragraph{Resolution Design}
Note that rule~$\DynRes$ is not as strong as it could be when purely
considering the logical interpretation of rules. In terms of proposition logic,
it does not allow to prove $A \rightarrow B$ from $A \rightarrow C$ and $C
\rightarrow B$. It only proves $A \rightarrow B$ from, e.g.,
$C \rightarrow B$ and $C$.
To obtain stronger resolution,  we would have to add $\pi$ as
a set of available assumptions to the environment:
\[ \myirule
{ \lookup{\tstate}{\type} = 
  \rclos{\rulesch{\beta}{\pi'}{\type'}, e', 
    \tstate', \rulepgmvar'} \\ 
  \rulet \leteq \rulesch{\alpha}{\pi}{\type} \quad
  \theta \leteq \unify{\type'}{\type}{\bar{\beta}} \\
  \tstate\shade{;\pi:\Box} \vturns \rulet_i \eval v_i \quad 
  (\forall \rulet_i \in \theta \pi')
}
{ \tstate \vturns \rulet \eval 
  \rclos{\rulet, \theta e', \theta \tstate', 
    \rulepgm \cup  \theta \rulepgmvar'}
} \]
However, there are two practical problems with that. Firstly, we do not have
any value-level evidence ($\Box$) for $\pi$ yet. Secondly and most importantly,
in this variant a query involves not one single environment
throughout, but many: a new one in every recursive resolution step.  This makes it
much harder to reason about safety and coherence properties, both for the
programmer and for an automatic type checker. For these two reasons, we have
decided to adopt the simpler resolution rule.
%-------------------------------------------------------------------------------
\subsection{Runtime Errors and Coherence Failures}
\label{subsec:error}
In $\ourlang$, ill-behaved programs either raise runtime errors or are
incoherent. The principal source of runtime errors is query failure,
which is caused by either lookup failure or ambiguous instantiation
during resolution. Coherence failure happens when a query in a
program does not have a single nearest match or its single nearest
match is not the one used at runtime.

\paragraph{Lookup Failures}
A lookup fails if there is no matching rule in the rule environment,
or there are multiple matching rules.

The first cause, no matching rule, is the simplest, illustrated by the
following two examples:
\[\begin{array}{rl}
\myset{} &\turns  \ensuremath{?\!\Conid{Int}} \\
\myset{\ensuremath{\{\mskip1.5mu \Conid{Bool}\mskip1.5mu\}\Rightarrow \Conid{Int}\mathbin{:}\mathbin{-}}}& \turns \ensuremath{?\!\Conid{Int}}
\end{array}
\noindent \]
In the first example, resolution does not find a matching rule for the
given \ensuremath{\Conid{Int}} type in the environment. In the second example,
resolution finds a matching rule for \ensuremath{\Conid{Int}} in the first step, but
does not find one in the recursive step for \ensuremath{\Conid{Bool}}.

The second cause are multiple matching rules, which is the case in the
following two examples:
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{3}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[3]{}\{\mskip1.5mu \Conid{Int}\mathbin{:}\mathrm{1},\Conid{Int}\mathbin{:}\mathrm{2}\mskip1.5mu\}\;\turns\;?\!\Conid{Int}{}\<[E]%
\\
\>[3]{}\{\mskip1.5mu \forall \alpha\hsforall \hsdot{\circ }{.}\alpha\to \Conid{Int}\mathbin{:}\mathbin{-},\forall \alpha\hsforall \hsdot{\circ }{.}\Conid{Int}\to \alpha\mathbin{:}\mathbin{-}\mskip1.5mu\}\;\turns\;?\!(\Conid{Int}\to \Conid{Int}){}\<[E]%
\ColumnHook
\end{hscode}\resethooks
\noindent

In the first example, two different rules produce a value for the same
type \ensuremath{\Conid{Int}}; arbitrarily choosing one of 1 and 2
makes the program's behavior unpredictable. To avoid this ambiguity,
the lookup fails instead. The second example shows that two rules can
be used to produce a value of the same type, even though the rule
types are different. The two polymorphic rule types can be instantiated to the
same type, in this case to \ensuremath{\Conid{Int}\to \Conid{Int}}.

\paragraph{Ambiguous Instantiations}
In some cases, resolution does not determine how to instantiate a
fetched rule. Consider the following example:\footnote{$\rclos{n}$
  denotes a closure value; distinct numbers mean distinct values.}\[
\begin{array}{rl}
  \myset{\quad 
    \ensuremath{\forall \alpha\hsforall \hsdot{\circ }{.}\{\mskip1.5mu \alpha\to \alpha\mskip1.5mu\}\Rightarrow \Conid{Int}\mathbin{:}\rclos{\mathrm{1}}} &, \\
    \ensuremath{\Conid{Bool}\to \Conid{Bool}\mathbin{:}\rclos{\mathrm{2}}}&, \\
    \ensuremath{\forall \beta\hsforall \hsdot{\circ }{.}\beta\to \beta\mathbin{:}\rclos{\mathrm{3}}}&} \turns \ensuremath{?\!\Conid{Int}}
\end{array}\]
% > { forall a. {a -> a} => Int : (rclos 1), Int -> Int : (rclos 2),
% >  Bool -> Bool : (rclos 3) } turns (query Int)
The \ensuremath{?\!\Conid{Int}} matches the first rule without determining an
instantiation for \ensuremath{\alpha}. However, the runtime behavior could actually
depend on the choice between \ensuremath{\rclos{\mathrm{2}}} and \ensuremath{\rclos{\mathrm{3}}}. Thus the query
is ambiguous.

\paragraph{Coherence Failures}
A program is coherent iff every query in the program has a single,
lexically nearest match, which is the same statically and at runtime. This
means that all the runtime queries instantiated from the original
query should have the same resolution result. Consider the following
example:
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{3}{@{}>{\hspre}l<{\hspost}@{}}%
\column{5}{@{}>{\hspre}l<{\hspost}@{}}%
\column{9}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[3]{}\mathbf{let}\;\Varid{f}\mathbin{:}\forall \beta\hsforall \hsdot{\circ }{.}\beta\to \beta\mathrel{=}{}\<[E]%
\\
\>[3]{}\hsindent{2}{}\<[5]%
\>[5]{}{\bf implicit}\;\{\mskip1.5mu \lambda\Varid{x}.\Varid{x}\mathbin{:}\forall \alpha\hsforall \hsdot{\circ }{.}\alpha\to \alpha\mskip1.5mu\}\;\mathbf{in}{}\<[E]%
\\
\>[5]{}\hsindent{4}{}\<[9]%
\>[9]{}?\!(\beta\to \beta){}\<[E]%
\ColumnHook
\end{hscode}\resethooks
\noindent
This program is coherent because no matter which type the type
variable \ensuremath{\beta} will have at runtime, the resolution results for all
those queries are the same (\ensuremath{\forall \alpha\hsforall \hsdot{\circ }{.}\alpha\to \alpha}). However, the following program is
incoherent:
\begin{hscode}\SaveRestoreHook
\column{B}{@{}>{\hspre}l<{\hspost}@{}}%
\column{3}{@{}>{\hspre}l<{\hspost}@{}}%
\column{5}{@{}>{\hspre}l<{\hspost}@{}}%
\column{8}{@{}>{\hspre}l<{\hspost}@{}}%
\column{9}{@{}>{\hspre}l<{\hspost}@{}}%
\column{E}{@{}>{\hspre}l<{\hspost}@{}}%
\>[3]{}\mathbf{let}\;\Varid{f}\mathbin{:}\forall \beta\hsforall \hsdot{\circ }{.}\beta\to \beta\mathrel{=}{}\<[E]%
\\
\>[3]{}\hsindent{2}{}\<[5]%
\>[5]{}{\bf implicit}\;\{\mskip1.5mu \lambda\Varid{x}.\Varid{x}\mathbin{:}\forall \alpha\hsforall \hsdot{\circ }{.}\alpha\to \alpha\mskip1.5mu\}\;\mathbf{in}{}\<[E]%
\\
\>[5]{}\hsindent{3}{}\<[8]%
\>[8]{}{\bf implicit}\;\{\mskip1.5mu \lambda\Varid{n}.\Varid{n}\mathbin{+}\mathrm{1}\mathbin{:}\Conid{Int}\to \Conid{Int}\mskip1.5mu\}\;\mathbf{in}{}\<[E]%
\\
\>[8]{}\hsindent{1}{}\<[9]%
\>[9]{}?\!(\beta\to \beta){}\<[E]%
\ColumnHook
\end{hscode}\resethooks
\noindent
There are two possible results for the query \ensuremath{?\!(\beta\to \beta)}
depending on the type of \ensuremath{\beta} at runtime. If the query is instantiated
by the substitution $\subst{\ensuremath{\beta}}{\ensuremath{\Conid{Int}}}$, then the nearest result is
\ensuremath{\Conid{Int}\to \Conid{Int}} and otherwise, \ensuremath{\forall \alpha\hsforall \hsdot{\circ }{.}\alpha\to \alpha} is the one.

Our static type system will safely reject such programs that can have
the aforementioned runtime errors or coherence failures.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../Main"
%%% End: 

